Semiclassical Approximations to Cosmological Perturbations

We apply several methods related to the WKB approximation to study cosmological perturbations during inflation, obtaining the full power spectra of scalar and tensor perturbations to first and to second order in the slow-roll parameters. We compare our results with those derived by means of other methods, in particular the Green's function method, and find agreement for the slow-roll structure. Scalar wave propagation on the Schwarzschild background is also considered.

==> appendice_WKB.tex <==
\chapter{Approssimazione WKB e Sviluppo adiabatico}
\label{WKB_vs_adia}

In questa appendice daremo un senso all'equivalenza tra l'approccio WKB classico
e lo sviluppo adiabatico. In particolare tale prova sar\`{a} data per
l'ordine adiabatico $2$.

\section{Espansione WKB}

Questa sezione presenta l'approssimazione WKB cos\`{\i} come si trova su diversi testi
dedicati alla meccanica quantistica \cite{davydov,messiah,landau} o ai metodi matematici di risoluzione dei
problemi fisici \cite{bender_orszag}. Per rimanere aderenti al testo utilizzeremo, dove possibile,
le stesse notazioni, omettendo indici e pedici superflui.

L'equazione di nostro interesse \`{e} della forma

\begin{equation}
    \delta^{2}\,\frac{d^{2}\,u(x)}{dx^{2}}=Q(x)\,u(x)
    \label{schr_eq}
\end{equation}

\noindent con $Q(x)$ monotona crescente che passa da valori negativi a valori positivi.

La soluzione per $\delta\rightarrow 0$ si pu\`{o} scrivere come

\begin{equation}
    u(x)=\exp{\left[\frac{1}{\delta}\,\sum_{n=0}^{\infty}\delta^{n}\,S_{n}(x)\right]}\;.
    \label{WKB_sol_app}
\end{equation}

\noindent Questa \`{e} la formula di partenza dalla quale si deriva l'approssimazione WKB
ad un determinato ordine.

Ponendo (\ref{WKB_sol_app}) in (\ref{schr_eq}) e troncando la serie ad un numero finito
di termini $L$, troviamo, eguagliando i termini nelle potenze di $\delta$,
 un sistema di equazioni differenziali nelle derivate di $S_{l}(x)$ con
$l$ compreso tra $0$ e $L$. Risolvendo tale sistema di equazioni differenziali determiniamo
le $S_{l}(x)$ di nostro interesse come funzioni delle derivate di $Q(x)$. I primi termini dello
sviluppo in (\ref{WKB_sol_app}) sono

\begin{equation}
    S_{0}(x)=\pm\,\int^{x}\sqrt{Q(t)}\,dt
    \label{S0_x}
\end{equation}

\noindent soluzione della cosidetta \emph{equazione eikonale}: $S_{0}'^{2}=Q(x)$
\footnote{Da qui l'apice indicher\`{a} la derivazione nella variabile considerata per $S_{j}$ e $Q$.}

\begin{equation}
    S_{1}(x)=-\,\frac{1}{4}\,\ln Q(x)
    \label{S1_x}
\end{equation}

\noindent soluzione della cosidetta \emph{equazione di trasporto}:
$2\,S_{0}'\,S_{1}'\,+\,S_{0}''=0$

\begin{equation}
    S_{2}(x)=\pm\,\int^{x}\left[\frac{Q''}{8\,Q^{3/2}}-\frac{5\,(Q')^{2}}{32\,Q^{5/2}}\right]\,dt
    \label{S2_x}
\end{equation}

\noindent e

\begin{equation}
    S_{3}(x)=-\frac{Q''}{16\,Q^{2}}+\frac{5\,(Q')^{2}}{64\,Q^{3}}\;.
    \label{S3_x}
\end{equation}

Scriviamo ora la soluzione al quart'ordine WKB (con $S_{0},S_{1},S_{2},S_{3}$)
raccogliendo i fattori comuni\footnote{In questa appendice l'ordine a cui ci si
riferisce per l'approssimazione WKB \`{e} da intendersi come il numero di termini $S_{j}$
che si considerano, partendo da $S_{0}$.}

\begin{equation}
    \begin{array}{ll}
    u^{(4)}_{wkb}(x)=e^{-\frac{1}{4}\,\ln Q(x)}\,
    \left\{A_{+}\,e^{\left[\frac{1}{\delta}\,\left(\int^{x}\sqrt{Q(t)}\,dt
    +\delta^{2}\,\int^{x}\left[\frac{Q''}{8\,Q^{3/2}}-\frac{5\,Q'^{2}}{32\,Q^{5/2}}\right]dt\right)\right]}
    \right.\\
    \\
    \left.\quad+A_{-}\,e^{\left[\frac{1}{\delta}\,\left(
    -\int^{x}\sqrt{Q(t)}\,dt
    -\delta^{2}\,\int^{x}\left[\frac{Q''}{8\,Q^{3/2}}-\frac{5\,Q'^{2}}{32\,Q^{5/2}}\right]dt\right)\right]}
    \right\}\,
    e^{\delta^{2}\,\left(-\frac{Q''}{16\,Q^{2}}+\frac{5\,Q'^{2}}{64\,Q^{3}}\right)}
    \end{array}
    \label{sol_WKB_4_racc}
\end{equation}

\noindent ora, con $\delta=1$ e semplificando ulteriormente

\begin{equation}
    \begin{array}{ll}
    u^{(4)}_{wkb}(x)=\frac{1}{\left[Q(x)\right]^{1/4}}\,
    \left\{A_{+}\,e^{\left[\int^{x}\left(\sqrt{Q(t)}\,
    +\frac{Q''}{8\,Q^{3/2}}-\frac{5\,Q'^{2}}{32\,Q^{5/2}}\right)dt\right]}
    \right.\\
    \\
    \left.\qquad\qquad\qquad+A_{-}\,e^{\left[-\,\int^{x}\left(\sqrt{Q(t)}\,
    +\frac{Q''}{8\,Q^{3/2}}-\frac{5\,Q'^{2}}{32\,Q^{5/2}}\right)dt\right]}
    \right\}\,
    e^{\left(-\frac{Q''}{16\,Q^{2}}+\frac{5\,Q'^{2}}{64\,Q^{3}}\right)}\;.
    \end{array}
    \label{sol_WKB_4_semp}
\end{equation}

\section{Sviluppo adiabatico}

Questa sezione presenta la tecnica dello sviluppo adiabatico al second'ordine come viene
presentata da Birrell e Davies in \cite{birrel}. La notazione che utiliziamo \`{e} quella del capitolo
\ref{WKB} omettendo le scritture non essenziali.

Come gi\`{a} indicato la soluzione formale all'ordine adiabatico $2$
\`{e} \footnote{Tralasciando la normalizzazione, inutile per lo scopo dell'appendice, ed indicando
anche la soluzione con il segno $+$ nell'esponenziale.}

\begin{equation}
    u^{(2)}(x)=\frac{1}{\sqrt{W^{(2)}(x)}}\,\left\{
    \widetilde{A}_{+}\,e^{\left[i\,\int^{x}W^{(2)}(t)\, dt\right]}
    +\widetilde{A}_{-}\,e^{\left[-\,i\,\int^{x}W^{(2)}(t)\, dt\right]}
    \right\}
    \label{WKB_formal_sol_2_app}
\end{equation}

\noindent con

\begin{equation}
    W^{(2)}(x)=\omega(x)\,\left[1+\sigma_{2}(x)\right]^{\frac{1}{2}}
    \label{W_2th_order_app}
\end{equation}

\noindent e

\begin{equation}
    \sigma_{2}=-\,\frac{1}{2}\,\frac{\ddot{\omega}}{\omega^{3}}
    +\frac{3}{4}\,\frac{\dot{\omega}^{2}}{\omega^{4}}\;.
    \label{sigma2j_app}
\end{equation}

Esplicitando in parte la scritura (\ref{WKB_formal_sol_2_app}) abbiamo

\begin{equation}
\begin{array}{ll}
    u^{(2)}(x)=\frac{1}{\sqrt{\omega(x)\,\left[1+\sigma_{2}(x)\right]^{\frac{1}{2}}}}\,\left\{
    \widetilde{A}_{+}\,e^{\left[i\,\int^{x}\omega(t)\,\left[1+\sigma_{2}(t)\right]^{\frac{1}{2}}\, dt\right]}
    \right.\\
    \\
    \left.\qquad\qquad\qquad\qquad\qquad\qquad+
    \widetilde{A}_{-}\,e^{\left[-\,i\,\int^{x}\omega(t)\,\left[1+\sigma_{2}(t)\right]^{\frac{1}{2}}\, dt\right]}
    \right\}\;.
\end{array}
    \label{WKB_formal_sol_2_app_esplic}
\end{equation}

Occorre ora dimostrare che le due formule (\ref{sol_WKB_4_semp}) e (\ref{WKB_formal_sol_2_app_esplic})
sono equivalenti ed in quali approssimazioni.

\section{Relazioni tra $Q(x)$ e $\omega(x)$}

Cominciamo con l'esprimere le funzioni di $Q(x)$ e delle sue derivate nella (\ref{sol_WKB_4_semp})
come funzioni di $\omega(x)$ e delle sue derivate. Sapendo che la nostra equazione \`{e}
\begin{equation}
    \frac{d^{2}u(x)}{dx^{2}}+\omega^{2}(x)\,u(x)=0
    \label{eq_moto_u_with_x_app}
\end{equation}

\noindent la riscriviamo nella forma di (\ref{schr_eq})

\begin{equation}
    \frac{d^{2}\,u(x)}{dx^{2}}=-\omega^{2}(x)\,u(x)
    \label{schr_eq_for_us}
\end{equation}

\noindent con $-\omega^{2}(x)$ anch'essa monotona crescente che passa da valori negativi
a valori positivi. Abbiamo quindi l'identificazione

\begin{equation}
    Q(x)=-\omega^{2}(x)\;.
    \label{identif}
\end{equation}

Possiamo identificare i termini che compaiono in (\ref{sol_WKB_4_semp})
\footnote{Qui gli apici ed i punti indicano sempre la derivazione in $x$ ma si preferisce adottarli
diversi rispettivamente per le derivate di $Q(x)$ e per le derivate di $\omega(x)$.}

\begin{equation}
    \sqrt{Q(x)}=i\,\omega(x)\;,
    \label{1st_id}
\end{equation}

\begin{equation}
    \frac{Q''}{8\,Q^{3/2}}-\frac{5\,Q'^{2}}{32\,Q^{5/2}}=i
    \left(\frac{3}{8}\,\frac{\dot{\omega}^{2}}{\omega^{3}}
    -\,\frac{1}{4}\,\frac{\ddot{\omega}}{\omega^{2}}\right)\;,
    \label{2nd_id}
\end{equation}

\begin{equation}
    -\frac{Q''}{16\,Q^{2}}+\frac{5\,Q'^{2}}{64\,Q^{3}}=
    \frac{1}{8}\,\frac{\ddot{\omega}}{\omega^{3}}
    -\,\frac{3}{16}\,\frac{\dot{\omega}^{2}}{\omega^{4}}\;.
    \label{3th_id}
\end{equation}

\section{Confronto}

Scriviamo ora la (\ref{sol_WKB_4_semp}) con $\omega(x)$ e la sue derivate

\begin{equation}
    \begin{array}{ll}
    u^{(4)}_{wkb}(x)=\frac{1}{\sqrt{i}\,\sqrt{\omega(x)}}\,
    \left\{A_{+}\,e^{\left[i\,\int^{x}\left(\omega(t)\,
    +\frac{3}{8}\,\frac{\dot{\omega}^{2}}{\omega^{3}}
    -\,\frac{1}{4}\,\frac{\ddot{\omega}}{\omega^{2}}\right)dt\right]}
    \right.\\
    \\
    \left.\qquad\qquad\qquad+A_{-}\,e^{\left[-\,i\,\int^{x}\left(\omega(t)\,
    +\frac{3}{8}\,\frac{\dot{\omega}^{2}}{\omega^{3}}
    -\,\frac{1}{4}\,\frac{\ddot{\omega}}{\omega^{2}}\right)dt\right]}
    \right\}\,
    e^{\left(\frac{1}{8}\,\frac{\ddot{\omega}}{\omega^{3}}
    -\,\frac{3}{16}\,\frac{\dot{\omega}^{2}}{\omega^{4}}\right)}
    \end{array}
    \label{sol_WKB_4_with_om}
\end{equation}

\noindent dove la radice di $i$ sar\`{a} riassorbita nella redefinizione della costanti $A_{\pm}$
che diventano $\widetilde{A}_{\pm}$.

Determiniamo quali altre approssimazioni occorrono per arrivare ad una completa identificazione tra (\ref{sol_WKB_4_with_om}) e (\ref{WKB_formal_sol_2_app_esplic}). Cominciamo con lo sviluppare
l'argomento dell'integrale in (\ref{WKB_formal_sol_2_app_esplic}) per piccoli $\sigma_{2}$
\footnote{Questo \`{e} lecito nel regime adiabatico.}

\begin{equation}
    W^{(2)}(x)=\omega(x)\,\left[1+\sigma_{2}(x)\right]^{\frac{1}{2}}
    \cong\omega(x)\,\left(1+\frac{1}{2}\,\sigma_{2}(x)\right)
    \label{W_2th_order_app_svil}
\end{equation}

\noindent ed anche

\begin{equation}
    \frac{1}{\sqrt{W^{(2)}(x)}}=\frac{1}{\sqrt{\omega(x)\,\left[1+\sigma_{2}(x)\right]^{\frac{1}{2}}}}
    \cong\frac{1}{\sqrt{\omega(x)}}\,\left(1-\frac{1}{4}\,\sigma_{2}(x)\right)\;.
    \label{W_2th_order_app_svil_freq}
\end{equation}

Sostituendo $\sigma_{2}$ abbiamo l'argomento dell'esponenziale

\begin{equation}
    W^{(2)}(x)
    \cong\omega(x)\,\left[1+\frac{1}{2}\,\left(-\,\frac{1}{2}\,\frac{\ddot{\omega}}{\omega^{3}}
    +\frac{3}{4}\,\frac{\dot{\omega}^{2}}{\omega^{4}}\right)\right]
    =\omega(x)-\,\frac{1}{4}\,\frac{\ddot{\omega}}{\omega^{2}}
    +\frac{3}{8}\,\frac{\dot{\omega}^{2}}{\omega^{3}}
    \label{W_2th_order_app_svil_sost}
\end{equation}

\noindent e

\begin{equation}
    \frac{1}{\sqrt{W^{(2)}(x)}}
    \cong\frac{1}{\sqrt{\omega(x)}}\,\left[1+\left(\frac{1}{8}\,\frac{\ddot{\omega}}{\omega^{3}}
    -\frac{3}{16}\,\frac{\dot{\omega}^{2}}{\omega^{4}}\right)\right]\;.
    \label{W_2th_order_app_svil_freq_sost}
\end{equation}

Riscriviamo la (\ref{WKB_formal_sol_2_app}) con quanto appena trovato

\begin{equation}
\begin{array}{ll}
    u^{(2)}(x)=\frac{\left[1+\left(\frac{1}{8}\,\frac{\ddot{\omega}}{\omega^{3}}
    -\frac{3}{16}\,\frac{\dot{\omega}^{2}}{\omega^{4}}\right)\right]}{\sqrt{\omega(x)}}\,\left\{
    \widetilde{A}_{+}\,e^{\left[i\,\int^{x}\left(\omega(t)-\,\frac{1}{4}\,\frac{\ddot{\omega}}{\omega^{2}}
    +\frac{3}{8}\,\frac{\dot{\omega}^{2}}{\omega^{3}}\right)\, dt\right]}\right.\\
    \\
    \left.\qquad\qquad\qquad\qquad\qquad
    +\widetilde{A}_{-}\,e^{\left[-\,i\,\int^{x}\left(\omega(t)-\,\frac{1}{4}\,\frac{\ddot{\omega}}{\omega^{2}}
    +\frac{3}{8}\,\frac{\dot{\omega}^{2}}{\omega^{3}}\right)\, dt\right]}
    \right\}\;.
\end{array}
    \label{WKB_formal_sol_2_app_sost}
\end{equation}

Ora per passare da $u^{(4)}_{wkb}$ a $u^{(2)}$ occorre sviluppare l'esponenziale che compare
nella soluzione WKB

\begin{equation}
    e^{\left(\frac{1}{8}\,\frac{\ddot{\omega}}{\omega^{3}}
    -\,\frac{3}{16}\,\frac{\dot{\omega}^{2}}{\omega^{4}}\right)}
    \cong1+\left(\frac{1}{8}\,\frac{\ddot{\omega}}{\omega^{3}}
    -\frac{3}{16}\,\frac{\dot{\omega}^{2}}{\omega^{4}}\right)\;.
    \label{svil_exp}
\end{equation}

Abbiamo mostrato che l'approssimazione WKB al quart'ordine e lo sviluppo adiabatico
al secondo coincidono a meno di termini di ordine superiore.

L'ordine adiabatico $0$ coincide con l'approssimazione WKB all'ordine $2$
(con $S_{0},S_{1}$ - approssimazione dell'ottica fisica),
come si vede immediatamente osservando le formule (\ref{sol_WKB_4_with_om}) e
(\ref{WKB_formal_sol_2_app_sost}) e tralasciando i termini in $\dot{\omega}$ e in
$\ddot{\omega}$ (ovvero senza considerare le correzioni $S_{2},S_{3}$ per la WKB
e $\sigma_{2}$ per lo sviluppo adiabatico).

\vspace{30cm}

$\phantom{\mu}$


==> bibliography.tex <==
%\pagestyle{headings}
%\begin{thebibliography}{99}
\bibliographystyle{unrst}
\bibliography{}
%
\bibitem{feynman}
R. Feynman, 
\emph{Feynman Lectures on Gravitation}
(p. 186, Addison-Wesley, US, 1995).
%
\bibitem{weinberg}
S. Weinberg,
\emph{Gravitation and Cosmology}
 (John Wiley \& Sons, New York, US, 1972).
%
\bibitem{KTbook}
E. W. Kolb and M. S. Turner,
\emph{The Early Universe}
( Addison-Wesley, US, 1990).
%
\bibitem{patridge}
R. B. Patridge,
\emph{3 K: the Cosmic Microwave Background Radiation}
(Cambridge University Press, Cambridge, UK, 1995).
%
\bibitem{zel1}
Ya. B. Zeldovich,
Sov. Phys. Usp. 6, 475 (1964)
[Usp. Fiz. Nauk. 80, 357 (1963)].
%
\bibitem{LK}
E. M. Lifshitz and I. M. Khalatnikov,
Sov. Phys. Usp. 6, 495 (1964)
[Usp. Fiz. Nauk. 80, 391 (1964)].
%
\bibitem{friedmann}
A. Friedmann,
Z. Phys. 10, 377 (1922);
Z. Phys. 21, 326 (1924).
%
\bibitem{lemaitre1}
G. Lema\^itre,
Ann. Soc. Sci. Bruxelles 47A, 49 (1927);
Rev. Questions Sci. 129, 129 (1958).
%
\bibitem{lemaitre2}
G. Lema\^itre,
Nature 128, 700 (1931).
%
\bibitem{eddington}
A. S. Eddington,
Month. Not. R. Astron. Soc. 90, 672 (1930).
%
\bibitem{KS}
H. Kodama and M. Sasaki,
Prog. Theor. Phys. Suppl. 78, 1 (1984).
%
\bibitem{sachs}
R. K. Sachs and A. M. Wolfe,
Astrophys. J. 147, 73  (1967).
%
\bibitem{sakharov}
A. D. Sakharov,
Sov. Phys. JETP 22, 241 (1965)
[Zh. Eksp. Teor. Fiz. 49, 345 (1965)].
%
\bibitem{silk1}
J. Silk, Nature 215, 1155 (1967);
Astrophys. J. 151, 459 (1968).
%
\bibitem{PeeblesYu}
P. J. E. Peebles and J. T. Yu,
Astrophys. J. 162, 815 (1970).
%
\bibitem{doro}
A. G. Doroshkevich, Ya. B. Zeldovich, and R. A. Sunyaev,
Sov. Astron. 22, 523 (1978).
%
\bibitem{wilson}
M. L. Wilson and J. Silk,
Astrophys. J. 243, 14 (1981).
%
\bibitem{cobe}
C. L. Bennet {\it et al.},
Astrophys. J. Lett. 464, L1 (1996).
%
\bibitem{cob2}
M. Tegmark,
Astrophys. J. Lett. 464, L35 (1996).
%
\bibitem{boom1}
de Bernardis {\it et al},
Astrophys. J. 564, 559 (2002).
%
\bibitem{boom2}
C. B. Netterfield {\it et al.},
Astrophys. J. 571, 604 (2002).
%
\bibitem{dasi}
N. W. Halverson {\it et al.},
Astrophys. J. 568, 38 (2002).
%
\bibitem{maxima}
A. T. Lee {\it et al.},
Astrophys. J. 561, L1 (2001).
%
\bibitem{archeops}
A. Beno\^it {\it et al.},
Astron. Astrophys. 399, L19 (2003).
%
\bibitem{silk}
E. Gawiser and  J. Silk,
Phys. Rept. 333, 245 (2000).
%
\bibitem{WMAP02}
 L. Page {\it et al},
Astrophys. J. Suppl.148, 223 (2003).
%
\bibitem{DICK}
C. Dickinson {\it et al},
Mon. Not. Roy. Astron. Soc. 353, 732 (2004).
%
\bibitem{mason}
B.S. Mason {\it et al},
Astrophys. J. 591, 540 (2003).
%
\bibitem{pearson}
T.J. Pearson {\it et al},
Astrophys. J. 591, 556 (2003).
%
\bibitem{kuo}
C.L. Kuo {\it et al},
Astrophys. J.  600, 32 (2004).
%
\bibitem{WMAP01}
C. L. Bennett {\it et al.},
Astrophys. J. Suppl. 148, 1 (2003).
%
\bibitem{LSS01}
M. Tegmark {\it et al.},
Astrophys. J. 606, 702 (2004).
%
\bibitem{CL01}
N. Bachall {\it et al.},
Astrophys. J. 585, 182 (2003).
%
\bibitem{BBN01}
B. Fields and S. Sarkar,
Phys. Lett. B 592, 202 (2004).
%
\bibitem{white}
M.J. White, D. Scott and J. Silk,
Ann. Rev. Astron. Astrophys. 32, 319 (1994).
%
\bibitem{dodelson}
W. Hu and S. Dodelson,
Ann. Rev. Astron. Astrophys. 40, 171 (2002).
%
\bibitem{bond}
J. R. Bond,
\emph{Cosmology and Large Scale Structure}
(eds. R. Schaeffer, J. Silk, M. Spiro and J. Zinn-Justin, p. 469, Les Houches, Session LX, 1993 ).
%
\bibitem{martin_sl_roll}
J. Martin, D.J. Schwarz,
Phys. Rev. D 62, 103520 (2000).
%
\bibitem{bardeen}
J.M. Bardeen,
Phys. Rev. D 22, 1882 (1980).
%
\bibitem{lythstewart}
D. H. Lyth and E. D. Stewart,
Phys. Lett. B 274, 168 (1992).
%
\bibitem{SL}
E.D. Stewart and D.H. Lyth,
Phys. Lett. B 302, 171 (1993).
%
\bibitem{martin_schwarz2}
J. Martin and D.J. Schwarz,
Phys. Rev. D 67, 083512 (2003).
%
\bibitem{H_MP}
S. Habib, K. Heitmann, G. Jungman and C. Molina-Par\'{\i}s,
Phys. Rev. Lett. 89, 281301 (2002).
%
\bibitem{mukh}
V.F. Mukhanov,
Sov. Phys. JETP Lett. 41, 493 (1985);
Sov. Phys. JETP Lett. 67, 1297 (1988).
%
\bibitem{mukh_thory}
V.F. Mukhanov, H.A. Feldman and R.H. Brandenberger,
Phys. Rep. 215, 203 (1992).
%
\bibitem{wang_mukh}
L. Wang, V.F. Mukhanov and P.J. Steinhardt,
Phys. Lett. B 414, 18 (1997).
%
\bibitem{SGong}
E.D. Stewart and J.O. Gong,
Phys. Lett. B 510, 1 (2001).
%
\bibitem{HHHJM}
S. Habib, A. Heinen, K. Heitmann, G. Jungman and C. Molina-Par\'{\i}s,
Phys. Rev. D 70, 083507 (2004).
%
\bibitem{olver}
F.W.J. Olver,
\emph{Asymptotics and special functions}
(AKP Classics, Wellesley, MA 1997).
%
\bibitem{birrel}
N.D. Birrel and P.C.W. Davies,
\emph{Quantum Fields in Curved Space}
(Cambridge University Press, Cambridge, England, 1982).
%
\bibitem{langer}
R.E. Langer,
Phys. Rev. 51, 669 (1937).
%
\bibitem{hunt}
P. Hunt and S. Sarkar,
Phys. Rev. D 70, 103518 (2004).
%
\bibitem{bender}
C.M. Bender and S.A. Orszag,
\emph{Advanced mathematical methods for scientists and engineers}
(McGraw-Hill Book Company, 1978).
%
\bibitem{schiff}
L.I. Schiff,
\emph{Quantum Mechanics}
(McGraw-Hill Book Company, 1952).
%
\bibitem{abram}
M. Abramowitz and I. Stegun,
\emph{Handbook of mathematical functions with formulas, graphs, and mathematical table}
(Dover Publishing, 1965).
%
\bibitem{langer49}
R.E. Langer,
Trans. Am. Math. Soc. 67, 461 (1949).
%
\bibitem{abbott}
L.F. Abbott and M.B. Wise,
Nucl. Phys. B 244, 541 (1984).
%
\bibitem{martin_PL}
J. Martin and D.J. Schwarz,
Phys. Rev. D 57, 3302 (1998).
%
\bibitem{WKB1}
R. Casadio, F. Finelli, M. Luzzi and G. Venturi,
Phys. Rev. D 71, 043517 (2005).
%
\bibitem{LLMS}
S.M. Leach, A.R. Liddle, J. Martin and D.J. Schwarz,
Phys. Rev. D 66, 023515 (2002).
%
\bibitem{lewin}
L. Lewin,
\emph{Dilogarithms and associated functions}
(Macdonald, 1958).
%
\bibitem{LPB}
A.R. Liddle, P. Parsons and J.D. Barrow,
Phys. Rev. D 50, 7222 (1994);
see also J.E. Lidsey, A.R. Liddle, E.W. Kolb, E.J. Copeland, T. Barreiro and M. Abney,
Rev. Mod. Phys. 69, 373 (1997).
%
\bibitem{hecht}
C.E. Hecht and J.E. Mayer,
Phys. Rev. 106, 1156 (1957).
%
\bibitem{mori}
H. Moriguchi,
J. Phys. Soc. Japan 14, 1771 (1959).
%
\bibitem{pechukas}
P. Pechukas,
J. Chem. Phys. 54, 3864 (1971).
%
\bibitem{MG}
S.C. Miller and R.H. Good,
Phys. Rev. 91, 174 (1953).
%
\bibitem{dingle}
R.B. Dingle,
Appl. Sci. Res. B 5, 345 (1956).
%
\bibitem{berry}
M.V. Berry and K.E. Mount,
Rep. Prog. Phys. 35, 315 (1972).
%
\bibitem{WKB_let}
R. Casadio, F. Finelli, M. Luzzi  and G.  Venturi,
Phys. Lett. B, 1 (2005).
%
\bibitem{WKB_SRprD}
R. Casadio, F. Finelli, M. Luzzi  and G.  Venturi,
Phys. Rev. D 72, 103516 (2005).
%
\bibitem{MCE}
R. Casadio, F. Finelli, A. Kamenshchik, M. Luzzi and G. Venturi,
JCAP 04, 011 (2006).
%
\bibitem{HHHJ}
S. Habib, A. Heinen, K. Heitmann and G. Jungman,
 Phys. Rev. D 71, 043518 (2005).
%
\bibitem{linde}
A.D. Linde,
Phys. Lett. B 129, 177 (1983).
%
\bibitem{BFV}
C. Bertoni, F. Finelli and G. Venturi,
Phys. Lett. A 237, 331 (1998).
%
\bibitem{FMVV_1}
F. Finelli, G. Marozzi, G.P. Vacca, and G.Venturi,
Phys. Rev. D 65, 103521 (2002).
%
\bibitem{KT}
A. Kosowsky and M.S. Turner,
Phys. Rev. D 52, 1739 (1995).
%
\bibitem{DeWitt}
B.S. DeWitt,
\emph{Dynamical theory of groups and fields}
(Gordon and Breach, New York, 1965).
%
\bibitem{Dinglebook}
R.B. Dingle,
\emph{Asymptotic expansions: their derivation and interpretation}
(Academic Press, London, 1973).
%
\bibitem{Ermakov}
V.P. Ermakov,
Univ. Izv. Kiev, series III 9, 1 (1880).
%
\bibitem{Pinney}
E. Pinney,
Proc. Amer. Math. Soc. 1, 681 (1950).
%
\bibitem{Grad}
I.S. Gradstein  and I.M. Ryzhik,
\emph{Tables of integrals, series and products},
(Academic Press, New York, 1980).
%
\bibitem{Lewis}
H. R. Lewis,
J. Math. Phys. 9, 1976 (1968).
%
\bibitem{Milne}
W.E. Milne,
Phys. Rev. 35, 863 (1930).
%
\bibitem{Espinosa}
P. Espinosa,
\emph{Ermakov-Lewis dynamic invariants with some applications},
(MS Thesis, Instituto de F\'{i}sica - Universidad de Guanajuato, Le\`{o}n, 2000).
%
\bibitem{Fano}
U. Fano  and A.R.P. Rau,
\emph{Atomic Collisions and Spectra},
(Academic Press, Orlando, 1986).
%
\bibitem{cosmology}
F. Finelli, G.P. Vacca  and G. Venturi,
Phys. Rev. D 58, 103514 (1998);
F. Finelli, A. Gruppuso  and G. Venturi,
Class. Quantum Grav. 16, 3923 (1999);
H. Rosu, P. Espinosa  and M. Reyes,
Nuovo Cim. B 114, 1435 (1999);
R.M. Hawkins  and J.E. Lidsey,
Phys. Rev. D 66, 023523 (2002).
%
\bibitem{Gray}
C. J. Eliezer and A. Gray,
SIAM J. Appl. Math. 30, 46 (1976).
%
\bibitem{ioffe}
M. V. Ioffe and H. J. Korsch,
Phys. Lett. A 311, 200 (2003).
%
\bibitem{Ray}
J. R. Ray and J.L. Reid,
Phys. Lett. A 71, 317 (1979).
%
\begin{comment}
%
\bibitem{weinb}  S. Weinberg;  \emph{Gravitation and Cosmology.}
John Wiley \& Sons, New York (1972).
%
\bibitem{einstein_1917} A. Einstein,
Sitz. Preuss. Akad. d. Wiss. (1917).
%
\bibitem{mis_tho_whee} C.W. Misner, K.S. Torne, J.A. Wheeler; \emph{Gravitation.}
Freeman, San Francisco (1973).
%
\bibitem{wald} R.M. Wald; \emph{General Relativity.}
The University of Chicago Press-Chicago and London (1984).
%
\bibitem{hubble} E. Hubble,
Proc. N.A.S. 15, 168 (1929).
%
\bibitem{penzias_wilson} A.A. Penzias, R.W. Wilson,
Astrophys. J. 142, 419 (1965).
%
\bibitem{guth} A.H. Guth,
Phys. Rev. D 23, 347 (1981).
%
\bibitem{freedman} W.L. Freedman \textit{et al.},
 arXiv:astro-ph/0012376.
%
\bibitem{bond} J.R. Bond \textit{et al.},
arXiv:astro-ph/0210007.
%
\bibitem{mather} J.C. Mather \textit{et al.},
Astrophys. J. 512, 511 (1999).
%
\bibitem{sachs_wolfe} R.K. Sachs, A.M. Wolfe,
Astrophys. J. 147, 73 (1967).
%
\bibitem{mukhanov_CMB-slow} V. Mukhanov,
arXiv:astro-ph/0303072.
%
\bibitem{BOOMERANG} P. De Bernardis \textit{et al.},
Nature 404, 955 (2000).
%
\bibitem{K_K_zoo} S. Dodelson, W.H. Kinney, E.W. Kolb,
Phys. Rev. D 56, 3207 (1997).
%
\bibitem{K_zoo} W.H. Kinney,
Phys. Rev. D 58, 123506 (1998).
%
\bibitem{riotto2} A. Riotto, V. Acquaviva, N. Bartolo, S. Matarrese,
 arXiv:astro-ph/0209156.
%
\bibitem{ger_par_liddle} A.R. Liddle, P. Parson, J.D. Barrow,
Phys. Rev. D 50, 7222 (1994).
%
\bibitem{mukhanov_var} V.F. Mukhanov,
Sov. Phys. JETP 68, 1297 (1988) [Zh. Eksp. Teor. Fiz. 94, 1-11 (July 1988)].
%
\bibitem{bardeen_turner} J.M. Bardeen, P.J. Steinhardt, M.S. Turner,
Phys. Rev. D 28, 679 (1983).
%
\bibitem{guth_pi} A.H. Guth, So-Y. Pi,
Phys. Rev. Lett. 49, 1110 (1982).
%
\bibitem{habib_molina-paris} S. Habib, K. Heitmann, G. Jungman, C. Molina-Par\'{\i}s,
Phys. Rev. Lett. 89, 281301 (2002).
%
\bibitem{VV_voce} G. Venturi, G. Vacca,
Comunicazioni personali.
%
\bibitem{nag_yok} M. Nagasawa, J. Yokoyama,
Nucl. Phys. B 370, 742.
%
\bibitem{chakraborty} B. Chakraborty,
J. Math. Phys. 14, 188 (1973).
%
\bibitem{marozzi_doc} G. Marozzi,
\emph{PHD Thesis} Unpublished (2003).
%
\bibitem{abramo_steg} M. Abramowitz, I.A. Stegun,
\emph{Handbook of Mathematical Funtions.}  Dover Publ. Inc. New York (1972).
%
\bibitem{davydov} A.S. Davydov,
\emph{Quantum Mechanics.}  Pergamon Press Ltd. London (1965).
%
\bibitem{messiah} A. Messiah,
\emph{M\'{e}canique quantique. Tome I.}  Dunod Paris (1969).
%
\bibitem{landau} L.D. Landau, E.M. Lifshitz,
\emph{Meccanica quantistica - teoria non relativistica.}  Editori Riuniti-Edizioni Mir (1976).
%
\bibitem{wmap}
http://wmap.gsfc.nasa.gov
%
\bibitem{sdss}
http://www.sdss.org
%
\bibitem{planck}
http://www.esa.int/science/planck
%
\bibitem{LLKCTBA}
J.E. Lidsey, A.R. Liddle, E.W. Kolb, E.J. Copeland, T. Barreiro and 
M. Abney, Rev. Mod. Phys. 69, 373 (1997).
%
\bibitem{TW}
N.C. Tsamis and R.P. Woodard, Class. Q. Grav. 20, 5205 (2003).
%
\bibitem{FMVV_II}
F. Finelli, G. Marozzi, G. P. Vacca, and G. Venturi, 
Phys. Rev. D 69, 123508 (2004).
%
\bibitem{gris}
L.P. Grishchuk, Sov. Phys. JETP Lett. 40, 409 (1974).
%
\bibitem{staro}
A. A. Starobinsky, JETP Lett. 30, 682 (1979).
%
\bibitem{terrero}
D.J. Schwarz, C.A. Terrero-Escalante and A.A. Garc\`{\i}a,
Phys. Lett. B 517, 243 (2001).
%
\bibitem{tesi}
M. Luzzi, {\em Laurea thesis} (unpublised, 2003).
%
\bibitem{langer34}
R.E. Langer, Bull. Am. Math. Soc. 40, 545 (1934).
%
\bibitem{polarski}
D. Polarski and A.A. Starobinsky,
Class. Quant. Grav. 13, 377 (1996).     
%
\bibitem{infla}
A.D. Linde, {\em Particle physics and inflationary cosmology}
(Harwood, Chur, Switzerland, 1990) arXiv:hep-th/0503203.
A.R. Liddle and D.H. Lyth, {\em Cosmological inflation and
large-scale structure} (Cambridge University Press, Cambridge,
England, 2000).
%
\bibitem{peiris}
H.V. Peiris et al.,
Ap. J. Suppl. Series, 148, 213 (2003).
%
\bibitem{PL}
F. Lucchin and S. Matarrese,
Phys. Rev. D 32, 1316 (1985).
%
\bibitem{pageetal}
L. Page et al.,
Ap. J. Suppl. Series, 148, 233 (2003).
%
\bibitem{cmb}
U. Seljak, N. Sugiyama, M.J. White and M. Zaldarriaga,
Phys. Rev. D 68,  083507 (2003).
%
\end{comment}
\end{thebibliography}

%\end{document}


==> review_methods.tex <==
\chapter{Soluzione delle equazioni per le perturbazioni}
\label{rev_met}

Scopo di questo capitolo \`{e} indicare i diversi metodi che negli ultimi dieci anni
sono stati proposti per la risoluzione delle equazioni delle perturbazioni
cosmologiche (eq. (\ref{eq_moto_mu_gen})). Qui non saranno indicati nel dettaglio i
conti effettuati da ciascun autore per pervenire al suo risultato; spesso non si
daranno nemmeno le formule finali degli spettri alle quali quest'ultimi approdano.
Questa scelta \`{e} dettata dal fatto di voler evitare confusione con le differenti
notazioni adottate e fornire semplicemente una spiegazione il pi\`{u} chiara possibile
dei diversi approcci senza entrare nei tecnicismi matematici adottati (per
approfondimenti si consiglia la lettura dei lavori originari, una referenza basilare
su cui si trovano indicazioni ulteriori \`{e} \cite{wang_mukh}).

Prima di iniziare questa presentazione riscriviamo le formule che abbiamo determinato nel
capitolo precedente, l'equazione del moto

\begin{equation}
    \frac{d^{2}\mu_{j}(\eta)}{d\eta^{2}}+\omega_{j}^{2}(k,\eta)\,\mu_{j}(\eta)=0\qquad j=S,T
    \label{eq_moto_mu_gen_rip}
\end{equation}

\noindent e la frequenza

\begin{equation}
    \omega_{j}^{2}(k,\eta)=k^{2}-U_{j}(\eta)=k^{2}-\frac{z_{j}''}{z_{j}}\qquad j=S,T\;.
    \label{freq_assump_rip}
\end{equation}

\section{Metodi esatti gauge-invarianti}

Il metodo rigoroso per determinare lo spettro di potenza primordiale sarebbe quello
di trovare una soluzione per l'equazione (\ref{eq_moto_mu_gen_rip}) per ogni
$\mu_{\boldsymbol{k},j}$ \footnote{Ricordiamo che con la (\ref{mu_assump}) abbiamo
tralasciato il $\boldsymbol{k}$ al pedice per semplificare la notazione.}, partendo
da quando la corrispondente lunghezza d'onda \`{e} piccola se comparata con
l'orizzonte, a quando essa lo supera \cite{mukhanov_var,bardeen_turner}. Un approccio
di questo tipo consiste nel risolvere un'equazione di un oscillatore armonico con
frequenza dipendente dal tempo. Nel caso generico non esiste una soluzione di questo
problema; specificando $a$ (quindi $H$ e tutti gli $\epsilon_{n}$) si esplicita la
 frequenza e si ha la possibilit\`{a} di trovare alcune forme che
permettano una soluzione analitica esatta. Questa circostanza \`{e} limitata a
pochissimi andamenti (De Sitter e legge di potenza \cite{riotto,abbott}) e pu\`{o} essere usata solamente per trovare
soluzioni esatte con cui confrontare risultati approssimati determinati con altri
metodi e testare la bont\`{a} di questi ultimi.

\section{Formalismo del Time-delay}

Questo metodo fu originariamente introdotto da Guth e Pi nel 1982 \cite{guth_pi} per
calcolare lo spettro delle perturbazioni di densit\`{a} d'energia alla fine
dell'inflazione. In quel modello si assumeva che l'inflazione fosse ben descritta da
una fase di De Sitter che si concludeva con una transizione istantanea ad una fase
idrodinamica. Gli aspetti fondamentali erano: (a) le perturbazioni della metrica
potevano essere completamente trascurate durante la fase di espansione esponenziale,
(b) il time-delay per perturbazioni con numero d'onda comovente $\boldsymbol{k}$,
definito come
$\delta\eta_{\boldsymbol{k}}:=\delta\varphi_{\boldsymbol{k}}(t)/\dot{\varphi}_{0}(t)$,
tendeva ad una quantit\`{a} indipendente dal tempo quando le perturbazioni venivano
``stirate'' ben al di l\`{a} dell'orizzonte, permettendo di recuperare, al termine
della fase di De Sitter, le perturbazioni della metrica.

Formalmente il metodo del time-delay non pu\`{o} essere esteso in modo rigoroso a
modelli qualsiasi, perch\`{e} vale

\begin{equation}
    \dot{H}=-\,4\,\pi\,G\,\dot{\varphi}_{0}^{2}
    \label{H.back}
\end{equation}

\noindent ottenuta riscrivendo la (\ref{Eins_acc}) usando (\ref{rho_phi_cl}) e
(\ref{p_phi_cl})\footnote{Occorre notare che la derivazione di questa relazione non
coinvolge ancora l'approssimazione di slow-roll.}. Da questa equazione emerge che nel
limite esatto di un'espansione alla De Sitter, per la quale vale $\dot{H}=0$, abbiamo
$\dot{\varphi}_{0}=0$ che porta alla divergenza di $\delta\eta_{\boldsymbol{k}}$.
Esiste per\`{o} un numero limitato di modelli per i quali questo formalismo offre
almeno un'indicazione dell'andamento dello spettro. Nell'approssimazione slow-roll e
nel limite per piccoli $\boldsymbol{k}$ (grandi lunghezze d'onda) la soluzione che
troviamo per $\delta\varphi$ all'equazione (\ref{KG_pert}) \`{e}

\begin{equation}
    \delta\varphi=C\,\frac{\left(\partial V/\partial\varphi\right)}{V}
    \label{varphi_sol}
\end{equation}

\noindent con $C$ costante. Ora, usando l'equazione di Friedmann
(\ref{Fried_eq_sl_roll}) e l'equazione del moto per $\varphi_{0}$
(\ref{eq_moto_phi0_sl_ro}), abbiamo

\begin{equation}
    \delta\eta=\frac{\delta\varphi}{\dot{\varphi}_{0}}=\frac{\tilde{C}}{\sqrt{V}}
    \label{time-delay_sol}
\end{equation}

\noindent dove $\tilde{C}$ \`{e} una nuova costante. Se $V$ dipende da
$\varphi_{0}(t)$ abbiamo un $\delta\eta$ dipendente dal tempo, inconsistente con il
criterio di applicabilit\`{a} del formalismo del time-delay. Avendo spesso a che fare
con potenziali $V$ dipendenti da $\varphi$, il time-delay si pu\`{o} considerare
solamente come approssimazione all'ordine pi\`{u} basso; la sua applicabilit\`{a} si
riduce ai soli potenziali estremamente piatti con $H$ circa costante su tutto
l'intervallo di e-foldings di interesse. Tra i modelli esclusi da queste costrizioni
vi sono la comune inflazione per legge di potenza (\emph{power law inflation})
e i modelli d'inflazione caotica.

\section{Approssimazione Horizon-Crossing/Bessel}

Questo metodo di approssimazione si basa su un approccio gauge-invariante esatto ma
evita l'integrazione diretta a $\boldsymbol{k}$ fissato (detta \emph{mode-by-mode}).
Sappiamo che l'ampiezza della perturbazione per un dato modo d'oscillazione
$\mu_{\boldsymbol{k},j}$, che rientra nell'orizzonte dopo l'epoca inflazionaria,
\`{e} espressa in termini dell'ampiezza che esso presentava al momento dell'uscita
dall'orizzonte durante l'inflazione. Per ottenere quest'ultima quantit\`{a} occorre
la soluzione crescente dell'equazione (\ref{eq_moto_mu_gen_rip}) nel limite di grandi
lunghezze d'onda $k^{2}\ll |z_{j}''/z_{j}|$, che \`{e} della forma

\begin{equation}
    \mu_{\boldsymbol{k},j}\cong C_{j}(k)\,z_{j}
    \label{long_w_sol}
\end{equation}

\noindent da connettere (farne il \emph{matching}) alla soluzione per piccole lunghezze d'onda
$k^{2}\gg |z_{j}''/z_{j}|$

\begin{equation}
    \mu_{\boldsymbol{k},j}\cong \frac{1}{\sqrt{2\,k}}\,e^{-\,i\,k\,\eta}\;.
    \label{short_w_sol}
\end{equation}

\noindent All'istante dell'attraversamento dell'orizzonte (da qui il nome \emph{horizon-crossing
approximation}) abbiamo $k=a\,H\,\mathcal{O}(1)$. Le condizioni di matching
determinano $C_{j}(k)$ da cui

\begin{equation}
    |C_{j}(k)|=\frac{\mathcal{O}(1)}{\sqrt{2\,k}\,z_{j}}
    \label{match}
\end{equation}

\noindent con $z_{j}$ valutata all'horizon-crossing. Lo spettro risulta quindi essere

\begin{equation}
    \mathcal{P}_{j}=f_{j}(H,\dot{\varphi})|_{k\,=\,a\,H}\,\mathcal{O}(1)
    \label{spectra}
\end{equation}

\noindent dove $f_{j}(H,\dot{\varphi})$ \`{e} una funzione diversa per $j=T,S$ e
valutata quando si ha esattamente $k=a\,H$. Il fatto di avere un $\mathcal{O}(1)$
rispecchia il problema della nostra conoscenza sullo spettro che stiamo cercando di
determinare; i diversi metodi proposti negli anni passati avevano, ed hanno ancora,
lo scopo di determinare tale funzione nel modo migliore possibile. L'approssimazione
di Bessel \`{e} un miglioramento dell'horizon-crossing, in quanto, invece di un
semplice matching a $k\sim a\,H$, usa come soluzione di (\ref{eq_moto_mu_gen_rip})
una funzione di Bessel nell'intorno di $k^{2}=|z_{j}''/z_{j}|$ e poi fa il matching
con i limiti gi\`{a} descritti sopra. La conoscenza accurata della soluzione in
questo regime di  lunghezze d'onda \`{e} molto importante, in quanto tale regione
\`{e} la pi\`{u} sensibile alla variazione nel tempo dei parametri di slow-roll che
guidano l'inflazione. La Bessel approximation ci offre quindi la possibilit\`{a} di
sostituire $\mathcal{O}(1)$ con funzioni dei parametri $\epsilon_{n}$. Ad una prima
analisi l'\emph{horizon-crossing/Bessel approximation} \footnote{Da qui in poi
la indicheremo con l'acronimo HC/BA.} sembra estendibile ad un grado di accuratezza
arbitrario. Tuttavia, come mostrato da Mukhanov, Wang e Steinhardt \cite{wang_mukh},
questa approssimazione non pu\`{o} essere portata ad ordini di correzione nei
parametri $\epsilon_{n}$ superiori al primo \cite{stewart_lyth_sl_roll,wang_mukh}.

Il motivo \`{e} il seguente: assumiamo che l'ampiezza di un dato modo d'oscillazione
sia determinata da un piccolo intervallo di e-folds attorno all'horizon-crossing; se
i parametri di slow-roll variano rapidamente in tale intorno l'assunzione appena
fatta cade. La condizione che gli $\epsilon_{n}$ (in particolare $\epsilon_{1}$)
cambino lentamente \`{e} necessaria ma non sufficiente perch\`{e} la HC/BA sia
valida. L'assunzione che $\epsilon_{1}$ sia costante\footnote{Come vedremo nel
prossimo capitolo $z_{j}''/z_{j}$ sar\`{a}, in opportune variabili che definiremo,
solamente funzione degli $\epsilon_{n}$.} (i successivi parametri slow-roll sono
nulli per (\ref{eps_eq_moto})) mi permette di determinare una soluzione esatta in
termini delle funzioni di Bessel. Occorre ricordare per\`{o} che l'ipotesi
$\epsilon_{1}=\textrm{cost}$ non \`{e} realistica per la cosmologia, poich\`{e} i parametri
di slow-roll devono ``avere la possibilit\`{a}'' di variare nel tempo in modo da far
terminare l'inflazione tornando all'espansione ordinaria. Considerando ora questi
parametri debolmente dipendenti dal tempo si incontra un problema nell'estensione
della HC/BA agli ordini superiori al primo; l'equazione non si risolve in termini
delle funzioni di Bessel perch\`{e} la frequenza che apparirebbe in esse
dipenderebbe dal tempo. Metodi che tentano di trattare funzioni di Bessel con frequenza
non costante sarebbero difficoltosi quanto la risoluzione dell'equazione esatta. Come
indicato in \cite{wang_mukh} si pu\`{o} comunque dare un'espressione al primo ordine
nei parametri di slow-roll.

Una prima classe di casi alla quale si pu\`{o} applicare tale metodo sono i modelli
del tipo new-inflation, inflazione caotica $\varphi^{n}$ con $n\gg 2$ e l'inflazione
estesa. Un ulteriore classe raccoglie modelli di natural-inflation, inflazione
caotica $\varphi^{n}$ con $n$ piccolo e alcuni modelli con due campi inflatonici. Per
quelli che non rientrano in tali schemi, l'applicazione di metodi di risoluzione
alternativi si rende indispensabile.

\section{Approssimazione dell'Orizzonte Costante}

Questo metodo, descritto da Schwarz, Terrero-Escalante e Garc\'{\i}a \cite{terrero},
si propone di utilizzare la HC/BA evitando le argomentazioni che ne impediscono
l'estensione ad ordini superiori al primo, imponendo vincoli sulla grandezza relativa
tra i diversi parametri di slow-roll. Tali costrizioni limitano ovviamente
l'applicabilit\`{a} del metodo ad un insieme pi\`{u} ristretto di potenziali. In
dettaglio i modelli ai quali si pu\`{o} applicare tale approccio sono quelli dove la
derivata nel tempo del parametro di Hubble $H$ \`{e} piccola, come per l'infalzione
vicino ad un massimo. Se $\epsilon_{1}\ll 1$ non si ha necessariamente che tutti gli
ordini in $\epsilon_{m}$ debbano essere piccoli, definiamo infatti la \emph{costant-horizon
approximation} (HCA) all'ordine $n$ con la richiesta
$|\epsilon_{2}^{n}|>\textrm{max}(|\epsilon_{1}\epsilon_{2}|,|\epsilon_{2}\epsilon_{3}|)$,
ci\`{o} significa che possiamo ora includere nel calcolo dello spettro primordiale
tutti i monomi del tipo:
$1,\,\epsilon_{1},\,\epsilon_{2},\,\epsilon_{2}^{2},\,\ldots\,\epsilon_{2}^{n}$.

\section{Approssimazione dell'Orizzonte Crescente}

Tale approccio presenta forti analogie con il metodo precedente \cite{terrero}. Le
conoscenze sul power-law inflation ($a\propto
t^{p}\rightarrow\epsilon_{1}=1/p=\textrm{cost}$ e $\epsilon_{m}=0$ per $m\geq 2$) ci
guidano nella definizione di questa approssimazione. Modelli inflazionari con
$|\epsilon_{m}|<\epsilon_{1}$ per $m\geq 2$ si possono approssimare prendendo tutti i
termini in $\epsilon_{1}$ fino all'ordine $n$, dove $n$ \`{e} il massimo intero per
cui vale
$|\epsilon_{1}^{n}|>\textrm{max}(|\epsilon_{1}\epsilon_{2}|,|\epsilon_{2}\epsilon_{3}|)$.
Per questi modelli $\epsilon_{1}\cong\textrm{cost}$ implica che $H$ vari al massimo
in modo lineare nel tempo. La \emph{growing-horizon approximation} (GHA) permette di
includere nel calcolo degli spettri i termini
$1,\,\epsilon_{1},\,\epsilon_{1}^{2},\,\ldots\,\epsilon_{1}^{n},\,\epsilon_{2}$. I
modelli che ricadono in questa tipologia sono quelli d'inflazione caotica $V\propto
\varphi^{p}$ con $p\,>\,4$.

\section{Metodo della funzione di Green}

Questo metodo \`{e} stato proposto nel 2001 da Stewart e Gong
\cite{stewart_gong_sl_roll}. La sua derivazione \`{e} piuttosto semplice. Si parte
dall'equazione originaria (\ref{eq_moto_mu_gen_rip}) e si definiscono una nuova
variabile

\begin{equation}
    x:=-\,k\,\eta
    \label{new_var}
\end{equation}

\noindent ed una nuova funzione

\begin{equation}
    y_{j}:=\sqrt{2\,k}\,\mu_{j}\;.
    \label{new_funct}
\end{equation}

L'equazione del moto diventa

\begin{equation}
    \frac{d^{2}y_{j}(x)}{dx^{2}}+\left(1-\,\frac{d^{2}z_{j}(x)/dx^{2}}{z_{j}(x)}\right)\,y_{j}(x)=0\qquad j=S,T\;.
    \label{new_eq_moto}
\end{equation}

\noindent Ora, occorre l'ansatz

\begin{equation}
    z_{j}(x):=\frac{1}{x}\,f_{j}(\ln x)
    \label{z_ansatz}
\end{equation}

\noindent dove $f_{j}(\ln x)$ \`{e} una funzione del logaritmo della nuova variabile.

Con quest'assunzione l'equazione (\ref{new_eq_moto}) risulta formalmente risolubile
utlizzando un'equazione integrale basata sulle funzioni di Green, accompagnata dalle
condizioni al contorno analoghe alle (\ref{long_w_sol}) e (\ref{short_w_sol}). Tale
strategia permette uno sviluppo perturbativo della soluzione ad un'ordine in linea di
principio arbitrario, senza incorrere nei problemi evidenziati per la HC/BA. Vincoli
sui modelli ai quali si pu\`{o} applicare tale procedura non esistono. I risultati
presentati in \cite{stewart_gong_sl_roll} si limitano a casi con un solo campo
inflatonico, ma l'estensione a modelli con pi\`{u} di un componente scalare che guida
l'inflazione risulta possibile.

\section{Approssimazione Uniforme}

Questa approsimazione \`{e} stata recentemente proposta da Habib \emph{et al.} \cite{habib_molina-paris}. Tale
approccio consiste nello scrivere l'equazione del moto (\ref{eq_moto_mu_gen_rip}) con
la definizione

\begin{equation}
    \frac{d^{2}z_{j}(\eta)/d\eta^{2}}{z_{j}(\eta)}=:\frac{\left(\nu_{j}^{2}(\eta)-1/4\right)}{\eta^{2}}\;.
    \label{nu_def}
\end{equation}

\noindent L'equazione assume la forma

\begin{equation}
    \frac{d^{2}\mu_{j}(\eta)}{d\eta^{2}}+\left[k^{2}-\,\frac{1}{\eta^{2}}\,\left(\nu_{j}^{2}(\eta)-1/4\right)\right]\,\mu_{j}(\eta)=0\qquad j=S,T\;.
    \label{habib_eq_moto_mu_gen}
\end{equation}

Nella HC/BA abbiamo che questa equazione pu\`{o} essere risolta senza incorrere in
problemi solamente se mantenuta al primo ordine nei parametri $\epsilon_{n}$. Con
questo nuovo metodo sarebbe possibile aggirare questo problema. L'\emph{approssimazione
uniforme} (UA) fornirebbe una soluzione che converge uniformemente per $\nu_{j}$
dipendente dal tempo. Secondo gli autori tale procedura pu\`{o} essere estesa
arbitrariamente agli ordini superiori. Vista l'estrema somiglianza con i risultati
che si ottengono con l'approssimazione WKB (che sar\`{a} presentata nel seguito) non
scendiamo ulteriormente nel dettaglio, anche alla luce di alcune critiche che pare si
possano portare a questo lavoro \cite{VV_voce} e nell'attesa di un'estensione dello stesso da parte
degli autori.

\vspace{0.5cm}

Un ulteriore metodo proposto per risolvere l'equazione (\ref{eq_moto_mu_gen_rip})
\`{e} quello dell'approssimazione WKB \cite{martin_schwarz}, ma tale tecnica sar\`{a}  presentata
in modo completo e sistematico nel prossimo capitolo.


==> wkb.tex <==
\chapter{Analysis of Cosmological Perturbations}
\label{WKB}
%
%
%
%
In this chapter we give the Wentzel-Kramers-Brillouin (WKB) approaches used to solve the equations that drive
the scalar and tensorial cosmological perturbations.
%
In first paragraph we conveniently redefine the problem and the power spectra,
then we briefly give the first application of WKB approximation to
cosmolgical perturbations~\cite{martin_schwarz2},
in the second one we present a first improved version of WKB analysis of
cosmological perturbations~\cite{WKB1}.
In the last paragraph we show a generalized WKB method, also called
Method of Comparison Equations~\cite{MCE}
%
%
%
\section{Standard WKB approximation}
\label{stWKB}
%
In this Section we begin by recalling that the straightforward
application of the standard WKB method leads to a poor
approximation and that the results can be improved to first adiabatic
order by means of the transformation~(\ref{transf}), as was shown in
Ref.~\cite{martin_schwarz2}.
However, the extension to higher orders is more subtle, as we shall
discuss in some detail.
\par
The WKB approximation is defined by first introducing a ``small''
parameter $\delta>0$ in order to perform the formal adiabatic
(or semiclassical) expansion of the mode
functions~\cite{birrel}~\footnote{Let us briefly recall that such
an expansion is called adiabatic when $\sqrt{\delta}$ is the
inverse of a (typically very large) time over which the system
evolves slowly, and semiclassical when $\sqrt{\delta}\sim\hbar$.}.
Consequently, Eqs.~(\ref{tensor_eq2}) and (\ref{scal_eq2})
[or equivalently Eqs.~(\ref{f_eqT}) and (\ref{f_eqS})] are formally replaced by
\be
\left[\delta\,\frac{\d^2}{\d\eta^2}+\Omega_j^2(k,\eta)\right]\,
\mu_j=0
\ ,
\label{eq_wkb_exp}
\ee
where
\be
\Omega_j^2(k,\eta)=k^2-\frac{z''_j}{z_j}
\ ,
\label{freq_eta}
\ee
with $j=S$ for scalar perturbations and $j=T$ for tensorial ones, so $z_S=z$ and $z_T=a$.
Redefining conveniently the power spectra of perturbations we can solve Eq.~(\ref{eq_wkb_exp})
together with the condition that the modes are initially plane waves for
wavelengths much shorter than the Hubble radius
%
\be
\lim_{\frac{k}{a\,H}\rightarrow +\infty} \mu(k,\eta)
=d\,\frac{{\rm e}^{-i\,k\,\eta}}{\sqrt{2\,k}}
\ ,
\label{init_cond_on_mu}
\ee
%
where $d=d_{\rm S}=1$ and $d=d_{\rm T}=\sqrt{8\,\pi}/m_{\rm Pl}$
for scalar and tensor perturbations ($m_{\rm Pl}$ is
the Planck mass~\footnote{We recall that $M_{\rm Pl}$ stand for the reduced Planck mass}).
So the dimensionless power spectra of scalar and tensor
fluctuations are given by the usual definitions
%
\be
\mathcal{P}_{\zeta}=
\displaystyle\frac{k^{3}}{2\,\pi^{2}}\,
\left|\frac{\mu_{\rm S}}{z_{\rm S}}\right|^{2}
\ ,
\ \
\mathcal{P}_{h}=
\displaystyle\frac{4\,k^{3}}{\pi^{2}}\,
\left|\frac{\mu_{\rm T}}{z_{\rm T}}\right|^{2}
\ .
\label{spectra_def}
\ee
%
The spectral indices and their runnings give the standard parametrization for the power spectra.
They are usually defined at an arbitrary pivot scale
$k_*$~\footnote{Sometimes the spectral indices and their runnings are
defined without the assumption $k=k_*$. In this work it is clear where we use this
assumption.} as
%
\be
n_{\rm S}-1=
\left.\displaystyle\frac{\d\ln \mathcal{P}_{\zeta}}
{\d\ln k}\right|_{k=k_{*}}
\ ,
\ \
n_{\rm T}=
\left.\displaystyle\frac{\d\ln \mathcal{P}_{h}}
{\d\ln k}\right|_{k=k_{*}}
\ ,
\label{n_def}
\ee
%
and
%
\be
\alpha_{\rm S}=\left.
\frac{\d^{2}\ln\mathcal{P}_{\zeta}}
{(\d\ln k)^{2}}\right|_{k=k_{*}}
\ ,
\ \
\alpha_{\rm T}=\left.
\frac{\d^{2}\ln \mathcal{P}_{h}}
{(\d\ln k)^{2}}\right|_{k=k_{*}}
\ .
\label{alpha_def}
\ee
%
We also define the tensor-to-scalar ratio
%
\be
R=\frac{\mathcal{P}_{h}}{\mathcal{P}_{\zeta}}
\ .
\label{Rat_def}
\ee
%
In the following we shall drop the subscript $j$, $S$ and $T$ if they are not necessary.
The limit $\delta\to 1$ must be taken at the end of the computation.
We then denote the leading order term in such an expansion
of $\mu$ by
%
\be
\mu_{{\rm WKB}}(k,\eta )=
\frac{{\rm e}^{\pm\frac{i}{\sqrt{\delta}}\,\int^{\eta }\Omega(k,\tau)
{\rm d}\tau}}{\sqrt{2\,\Omega(k,\eta)}}
\ ,
\label{wkb_sol}
\ee
%
which satisfies the following differential equation
%
\be
\left[\delta\,\frac{\d^2}{\d \eta^2}
+\Omega^2(k,\eta)-\delta\,Q_\Omega(k,\eta)\right]\,
\mu_{{\rm WKB}}=0
\ ,
\label{eq_wkb}
\ee
%
where
%
\be
Q_\Omega(k,\eta)\equiv
\frac{3}{4}\,\frac{(\Omega')^2}{\Omega^2}
-\frac{\Omega''}{2\,\Omega}
\ .
\label{Q}
\ee
%
We now observe that $\mu_{{\rm WKB}}$ is the exact solution of
Eq.~(\ref{eq_wkb_exp}) in the ``adiabatic limit'' $\delta\to 0$,
and is expected to be a good approximation to the exact $\mu$
(in the limit $\delta\to 1$) if
%
\be
\Delta\equiv
\left\vert\frac{Q_\Omega}{\Omega^2}\right\vert
\ll 1
\ .
\label{WKB_cond}
\ee
%
\par
On using the potentials in Eqs.~(\ref{tens_pot}) and (\ref{scal_pot}) in terms of
$a$ and $H$, one finds
%
\be
\Delta_{\rm S,T}=
\left\{ \begin{array}{ll}
\displaystyle\left(\frac{a\,H}{k}\right)^{4}
\mathcal{O}(\epsilon_{n})\sim 0
&
\textrm{sub-horizon scales}
\\
&
\\
\displaystyle\frac{1}{8}+\mathcal{O}(\epsilon_{n})\
&
\textrm{super-horizon scales.}
\end{array}
\right.
\label{cond_prechange}
\\
\nonumber
\ee
%
The result for super-horizon scales suggests that a change of
variable and function are necessary in order to obtain better
accuracy.
\par
A convenient change of dependent variable and funtion is the
Langer transformation~\cite{langer}
%
\be
x\equiv\ln\left(\frac{k}{H\,a}\right)
\ ,\quad
\chi\equiv(1-\epsilon_1)^{1/2}\,{\rm e}^{-x/2}\,\mu
\ ,
\label{transf}
\ee
%
introduced in Ref.~\cite{wang_mukh} is used~\footnote{Note
that we define $x$ with the opposite sign with respect to that in
Ref.~\cite{martin_schwarz2}.
This of course implies that our $x_i\to+\infty$ and $x_f\to-\infty$,
whereas $x_i\to-\infty$ and $x_f\to+\infty$ in
Ref.~\cite{martin_schwarz2}.}
in order to improve the accuracy.
Such a transformation bring Eqs.~(\ref{tensor_eq2}) and (\ref{scal_eq2})
into the form
%
\be
\left[\frac{{\d}^2}{{\d} x^2}+\omega^2(x)\right]
\,\chi=0
\ ,
\label{new_eq}
\ee
%
where the (new) frequency $\omega(x)$ in general vanishes at
the classical ``turning point'' $x=x_0$. In fact, on employing
the transformation (\ref{transf}), one finds (for $\delta=1$)
the new equations of motion (\ref{new_eq}), which explicitly read
%
{\footnotesize
\be
&&\!\!\!\!\!\!\!\!\!\!\!\!
\frac{\d^2\chi_{\rm S}}{\d x^2}
+\!\!\left[\frac{{\rm e}^{2\,x}}{(1-\epsilon_1)^2}
-\left(\frac{3-\epsilon_1}{2-2\,\epsilon_1}\right)^2
-\frac{(3-2\,\epsilon_1)\,\epsilon_2}{2\,(1-\epsilon_1)^2}
-\frac{(1-2\,\epsilon_1)\,\epsilon_2\,\epsilon_3}{2\,(1-\epsilon_1)^3}
-\frac{(1-4\,\epsilon_1)\,\epsilon_2^2}{4\,(1-\epsilon_1)^4} \right]\,
\chi_{\rm S}=0
\nonumber
\\
\label{eqST_x}
\\
&&\!\!\!\!\!\!\!\!\!\!\!\!
\frac{\d^2 \chi_{\rm T}}{\d x^2}
+\!\!\left[\frac{{\rm e}^{2\,x}}{(1-\epsilon_1)^2}
+\left(\frac{3-\epsilon_1}{2-2\epsilon_1}\right)^2
+\frac{\epsilon_1\,\epsilon_2}{2\,(1-\epsilon_1)^2}
+\frac{\epsilon_1\,\epsilon_2\,\epsilon_3}{2\,(1-\epsilon_1)^3}
+\frac{(2+\epsilon_1)\,\epsilon_1\,\epsilon_2^2}{4\,(1-\epsilon_1)^4}
\right]\,
\chi_{\rm T}=0
\nonumber
\ .
\ee
}
%
From $\omega_{\rm S}^2(x)$ and $\omega_{\rm T}^2(x)$, respectively
given by the expressions in the square brackets of
Eqs.~(\ref{eqST_x}), we now obtain
%
{\small
\be
\left\{\begin{array}{ll}
\!\!\!\Delta_{\rm S,T}
\!=\!e^{-2\,x}\mathcal{O}(\epsilon_{n})\sim 0
&
%\quad
\textrm{sub-horizon scales}
\\
\\
\!\!\!\Delta_{\rm S}
\!=\!\displaystyle\frac{4}{27}\,
\left(\epsilon_{1}\,\epsilon_{2}^2
+\epsilon_{1}\,\epsilon_{2}\,\epsilon_{3}+
\frac{\epsilon_{2}\,\epsilon_{3}^2}{2}
+\frac{\epsilon_{2}\,\epsilon_{3}\,\epsilon_{4}}{2}\right)
+\mathcal{O}(\epsilon_{n}^{4})
&
%\quad
\textrm{super-horizon scales}
\\
\\
\!\!\!\Delta_{\rm T}
\!=\!\displaystyle\frac{4}{27}\,
\left(\epsilon_{1}\,\epsilon_{2}^2
+\epsilon_{1}\,\epsilon_{2}\,\epsilon_{3} \right)
+\mathcal{O}(\epsilon_{n}^{4})
&
%\quad
\textrm{super-horizon scales}
\ ,
\end{array}
\right.
\label{rapp_Q/omega2}
\ee
}
%
and it is thus obvious that $\Delta$ becomes very small for any
inflationary potential satisfying the slow-roll
conditions~\cite{wang_mukh} in both limits of interest
(but, remarkably, not at the turning point).
As a consequence, the WKB approximation is now also valid on
super-horizon scales.
\par
One might naively expect that the transformation~(\ref{transf})
will improve the WKB approach to all orders (in the formal
expansion in $\delta$), thus yielding increasingly
better results.
However, since $Q$ diverges at the turning point $x=x_0$,
whether the function $\mu_{\rm WKB}$ can still be regarded
as a solution to Eq.~(\ref{eq_wkb_exp}) for $x\sim x_0$ in
the adiabatic limit $\delta\to 0$ becomes a subtle issue.
It is precisely for this reason that one usually considers
particular solutions around the turning point (for example,
combinations of Airy functions for a linear turning point)
which must then be matched with the asymptotic
form~(\ref{wkb_sol}) on both sides of the turning point.
The problem with this standard procedure is that there is no
general rule to determine the actual matching points
(which cannot be $x_0$ where $Q$ diverges) in such a way that
the overall error be small.
As a consequence, the standard adiabatic expansion for
$\delta\ll 1$ may not lead to a reliable approximation
around the turning point, which would then result in large
errors to higher orders and a questionable further
extension of all the expressions to the interesting case
$\delta=1$.
\par
It was in fact shown in Ref.~\cite{hunt} that a simple
extension to higher orders of the above procedure~\cite{bender}
actually seems to reduce the accuracy with respect to the
leading order results of~Ref.~\cite{martin_schwarz2}.
We shall see in the next Section that one can overcome this
problem by introducing mode functions which remain good
approximations also around the turning point.
%
%
%
\section{The ``Turning Point'' problem}
\label{TPproblem}
%
FFYVCV GFTYV YV F T F V76
%
%
%
\section{Improved WKB approximation}
\label{imprWKB}
%
We shall now describe a method to improve the WKB approximation
to all orders by following the scheme outlined in Ref.~\cite{langer}
(see also Ref.~\cite{schiff}).
The basic idea is to use approximate expressions which are valid
for all values of the coordinate $x$ and then expand around them.
Two different such expansions we shall consider, namely
one based on the Green's function technique and the other
on the usual adiabatic expansion~\cite{langer}.
\par
Let us first illustrate the main idea of Ref.~\cite{langer}
for the particular case $\omega^{2}=C\,\left(x-x_0\right)^{n}$,
with $C$ a positive costant.
All the solutions to Eq.~(\ref{new_eq}) for $x>x_0$ can be written
as linear combinations of the two functions
%
\be
u_{\pm}(x)=\sqrt{\frac{\xi(x)}{\omega(x)}}\,
J_{\pm m}\left[\xi(x)\right]
\ ,
\label{particular_sol}
\ee
%
where
%
\be
\xi(x)\equiv\int_{x_0}^{x}\omega(y)\,\d y
\ ,
\quad
\quad
m=\frac{1}{n+2}
\ ,
\label{xi_and_m}
\ee
and $J_\nu$ are Bessel functions~\cite{abram}.
Moreover, for a general frequency $\omega$,
the expressions in Eq.~(\ref{particular_sol})
satisfy
%
\be
\left[\frac{{\d}^2}{{\d} x^2}+\omega^2(x)-\sigma(x)\right]
\,u_{\pm}=0
\ ,
\label{eq_with_eta}
\ee
%
where the quantity (primes from here on will denote
derivatives with respect to the argument of the given
function)
%
\be
\sigma(x)
%&=&
=
\frac{3}{4}\,\frac{(\omega')^2}{\omega^2}
-\frac{\omega''}{2\,\omega}
+\left(m^{2}-\frac14\right)\,\frac{\omega^{2}}{\xi^{2}}
%\nonumber\\&=&
=
Q_\omega+\left(m^{2}-\frac14\right)\,\frac{\omega^{2}}{\xi^{2}}
\ ,
\label{sigma}
\ee
%
contains the term $Q$ defined in Eq.~(\ref{Q}),
whose divergent behavior at the turning point $x=x_0$ we
identified as the possible cause of failure of the standard WKB
approach.
For a general (finite) frequency, which can be expanded in powers
of $x-x_0$~\footnote{In the following we shall consider the
general case in Eq.~(\ref{omega_expand}), although one might restrict
to $n=1$, since our frequencies exhibit a linear turning point.},
%
\be
\omega^{2}(x)=C\,\left(x-x_0\right)^{n}
\left[1+\sum_{q\ge 1}\,c_q\,(x-x_0)^q\right]
\ ,
\label{omega_expand}
\ee
%
one finds that the extra term in Eq.~(\ref{sigma}) precisely
``removes'' the divergence in $Q$ at the turning point.
In fact, the residue
%
\be
\lim_{x\to x_0}\sigma(x)=\frac{3\,(n+5)\,c_1^{2}}{2\,(n+4)\,(n+6)}
-\frac{3\,c_2}{n+6}
\ ,
\label{limit_eta_at_TP}
\ee
%
is finite~\cite{langer,schiff}.
The finiteness of $\sigma$ at the turning point is crucial in
order to extend the WKB method to higher orders
(this point was missed in Ref.~\cite{hunt}).
It is also easy to show that, for the cases of interest,
$|\sigma/\omega^2|\simeq\Delta$ as given in
Eq.~(\ref{rapp_Q/omega2}) for $x\to\pm\infty$, so that
the new approximate solutions remain very accurate
for large $|x|$.
For slowly varying frequencies, with $|\sigma(x)|$ small
everywhere, the functions~(\ref{particular_sol}) are thus
expected to be good approximations to the solutions of
Eq.~(\ref{new_eq}) for the whole range of $x$, including
the turning point.
\par
We can now introduce both the adiabatic expansion of the previous
Section and a new formal expansion of the mode functions by
replacing Eq.~(\ref{new_eq}) by
%
\be
\left[\delta\,\frac{{\d}^2}{{\d} x^2}+
\omega^2(x)-\delta\,\sigma(x)\right]\,\chi
=-\delta\,\varepsilon\,\sigma(x)\,\chi
\ ,
\label{new_eq_rewrite}
\ee
%
where $\delta$ and $\varepsilon$ are ``small'' positive
parameters.
We shall refer to expressions proportional to $\delta^n$ as
the $n$-th adiabatic order and to those proportional to
$\varepsilon^n$ as the $n$-th perturbative order.
\par
It is convenient to consider the solutions to
Eq.~(\ref{new_eq_rewrite}) to the left and right of the
turning point $x_0$ separately.
We shall call:
\begin{subequations}
%
\begin{description}
\item[region~I)]
where $\omega^{2}>0$ (on the right of $x_0$), with
\be
\omega_{\rm I}(x)\equiv\sqrt{\omega^{2}(x)}
\ ,
\quad
\xi_{\rm I}(x)\equiv\int_{x_0}^{x}\omega_{\rm I}(y)\,\d y
\ ,
\label{xi_I}
\ee
and the solutions to the corresponding homogeneous equation
(\ref{eq_with_eta}) are given in Eq.~(\ref{particular_sol});
%
\item[region~II)]
where $\omega^{2}<0$ (on the left of
$x_0$), with
\be
\omega_{\rm II}(x)\equiv\sqrt{-\omega^{2}(x)}
\ ,
\quad
\xi_{\rm II}(x)\equiv\int_{x}^{x_0}\omega_{\rm II}(y)\,\d y
\ ,
\label{xi_II}
\ee
and the solutions to the corresponding homogeneous equation
(\ref{eq_with_eta}) are obtained from those in
Eq.~(\ref{particular_sol}) by replacing the $J_\nu$ with the $I_\nu$~\cite{abram}.
%
\end{description}
%
\end{subequations}
Corresponding expressions are obtained for all relevant
quantities, for example $\sigma_{\rm I}$ and $\sigma_{\rm II}$,
and we shall omit the indices I and II whenever it is not
ambiguous.
\par
Although it is possible to expand in both parameters,
so as to obtain terms of order $\delta^p\,\varepsilon^q$
(with $p$ and $q$ positive integers),
in the following we shall just consider each expansion separately,
that is we shall set $\delta=1$ in the perturbative expansion
(see~Section~\ref{pert}) and $\varepsilon=1$ in the adiabatic
expansion (see~Section~\ref{adiab}).
%
\subsection{Perturbative expansion}
\label{pert}
%
For $\delta=1$, the limit $\varepsilon\to 0$ is exactly solvable
and yields the solutions (\ref{particular_sol}), whereas the case
of interest (\ref{new_eq}) is recovered in the limit
$\varepsilon\to 1$, which must always be taken at the end of
the computation.
The solutions to Eq.~(\ref{new_eq_rewrite}) can be further
cast in integral form as
%
\be
\chi(x)=u(x)-\varepsilon\,\int G(x,y)\,\sigma(y)\,\chi(y)\,\d y
\ ,
\label{complete_sol}
\ee
%
where $u(x)=A_+\,u_{+}(x)+A_-\,u_{-}(x)$ is a linear combination
of solutions (\ref{particular_sol}) to the corresponding homogeneous
equation~(\ref{eq_with_eta}), and $G(x,y)$ is the Green's function
determined by
%
\be
\left[\frac{{\d}^2}{{\d} x^2}+\omega^2(x)-\sigma(x)\right]
\,G(x,y)
=\varepsilon\,\delta(x-y)
\ .
\label{green_eq}
\ee
%
The solutions of the homogeneous equation~(\ref{eq_with_eta})
in the two regions are then given by
%
{\small
\be
&&
\!\!\!\!\!\!\!\!\!\!u_{\rm I}(x)=
\displaystyle\sqrt{\frac{\xi_{\rm I}(x)}{\omega_{\rm I}(x)}}\,
\left\{
A_{+}\,J_{+m}\left[\xi_{\rm I}(x)\right]
+A_{-}\,J_{-m}\left[\xi_{\rm I}(x)\right]
\right\}
%\nonumber\\&\!\!\!\equiv\!\!\!&
\!\equiv\!
A_+\,u_{{\rm I}+}(x)+A_-\,u_{{\rm I}-}(x)
\nonumber
\\
\label{sol_in}
\\
&&
\!\!\!\!\!\!\!\!\!\!u_{\rm II}(x)=
\displaystyle\sqrt{\frac{\xi_{\rm II}(x)}{\omega_{\rm II}(x)}}\,
\left\{
B_{+}\,I_{+m}\left[\xi_{\rm II}(x)\right]
+B_{-}\,I_{-m}\left[\xi_{\rm II}(x)\right]
\right\}
%\nonumber\\&\!\!\!\equiv\!\!\!&
\!\equiv\!
B_+\,u_{{\rm II}+}(x)+B_-\,u_{{\rm II}-}(x)
\nonumber
\ee
}
%
and the Green's functions can be written as
%
\be
&&
\!\!\!\!\!\!\!\!\!\!\!\!\!\!G_{\rm I}(x,y)=
-\displaystyle\frac{\pi}{\sqrt{3}}\,
\theta(x-y)\,u_{{\rm I}-}(x)\,u_{{\rm I}+}(y)
%\nonumber\\&&
-\displaystyle\frac{\pi}{\sqrt{3}}\,
\theta(y-x)\,u_{{\rm I}+}(x)\,u_{{\rm I}-}(y)
\nonumber
\\
\label{green_funct}
\\
&&
\!\!\!\!\!\!\!\!\!\!\!\!\!\!G_{\rm II}(x,y)=
\displaystyle\frac{i\,\pi}{\sqrt{3}}\,
\theta(x-y)\,u_{{\rm II}-}(x)\,u_{{\rm II}+}(y)
%\nonumber\\&&
+\,\displaystyle\frac{i\,\pi}{\sqrt{3}}\,
\theta(y-x)\,u_{{\rm II}+}(x)\,u_{{\rm II}-}(y)
\ .
\nonumber
\ee
\par
With the ansatz
%
\be
\!\!\!\!\!\!\!\!\!\!
\chi_{\rm I}(x)&\!\!=\!\!&
A_{+}\,a_{+}(x)\,u_{{\rm I}+}(x)
+A_{-}\,a_{-}(x)\,u_{{\rm I}-}(x)
\nonumber
\\
\label{ansatz}
\\
\!\!\!\!\!\!\!\!\!\!
\chi_{\rm II}(x)&\!\!=\!\!&
B_{+}\,b_{+}(x)\,u_{{\rm II}+}(x)
+B_{-}\,b_{-}(x)\,u_{{\rm II}-}(x)
\ ,
\nonumber
\ee
%
from Eqs.~(\ref{sol_in}) and~(\ref{green_funct}),
the problem is now reduced to the determination
of the $x$-dependent coefficients
\be
&&
\!\!\!\!\!\!\!\!\!\!
a_{+}(x)\equiv\left[1+\varepsilon\,J^+_{+-}(x,x_i)\right]
+\varepsilon\,\frac{A_{-}}{A_+}\,J^-_{--}(x,x_i)
\nonumber
\\
\nonumber
\\
&&
\!\!\!\!\!\!\!\!\!\!
a_{-}(x)\equiv
\left[1+\varepsilon\,J^-_{+-}(x_0,x)\right]
+\varepsilon\,\frac{A_{+}}{A_-}\,J^+_{++}(x_0,x)
\nonumber
\\
\label{Abar_Bbar}
\\
&&
\!\!\!\!\!\!\!\!\!\!
b_{+}(x)\equiv
\left[1-i\,\varepsilon\,I^+_{+-}(x,x_0)\right]
-i\,\varepsilon\,\frac{B_{-}}{B_+}\,I^-_{--}(x,x_0)
\nonumber
\\
\nonumber
\\
&&
\!\!\!\!\!\!\!\!\!\!
b_{-}(x)\equiv
\left[1-i\,\varepsilon\,I^-_{+-}(x_f,x)\right]
-i\,\varepsilon\,\frac{B_{+}}{B_-}\,I^+_{++}(x_f,x)
\ ,
\nonumber
\ee
in which, for the sake of brevity (and clarity),
we have introduced a shorthand notation for the following
integrals
\be
%&&
\!\!\!\!\!\!\!\!\!\!
J^{w}_{s\bar s}(x_1,x_2)&\equiv&
\displaystyle\frac{\pi}{\sqrt{3}}\,
\int_{x_1}^{x_2}
\sigma_{\rm I}(y)\,a_w(y)\,
u_{{\rm I}s}(y)\,u_{{\rm I}\bar s}(y)\,\d y
\nonumber
\\
%&&\!\!\!\!\!\!\!\!\!\!
&=&
\displaystyle\frac{\pi}{\sqrt{3}}\,\int_{x_1}^{x_2}
\!\!\!\!
\sigma_{\rm I}(y)
\,\frac{\xi_{\rm I}(y)}{\omega_{\rm I}(y)}\,a_{w}(y)\,
\,J_{sm}\left[\xi_{\rm I}(y)\right]\,J_{\bar sm}\left[\xi_{\rm I}(y)\right]
\d y
\nonumber
\\
\phantom{A}
\\
%&&
\!\!\!\!\!\!\!\!\!\!
I^{w}_{s\bar s}(x_1,x_2)&\equiv&
\displaystyle\frac{\pi}{\sqrt{3}}\,
\int_{x_1}^{x_2}
\sigma_{\rm II}(y)\,b_w(y)\,
u_{{\rm II}s}(y)\,u_{{\rm II}\bar s}(y)
\,\d y
\nonumber
\\
%&&\!\!\!\!\!\!\!\!\!\!\!\!
&=&
\displaystyle\frac{\pi}{\sqrt{3}}\,\int_{x_1}^{x_2}
\!\!\!\!
\sigma_{\rm II}(y)
\,\frac{\xi_{\rm II}(y)}{\omega_{\rm II}(y)}\,b_{w}(y)\,
\,I_{sm}\left[\xi_{\rm II}(y)\right]\,
I_{\bar sm}\left[\xi_{\rm II}(y)\right]
\d y
\, ,
\nonumber
\ee
where the symbols $w$, $s$ and $\bar s$ are $+$ or $-$.
\par
Before tackling this problem, we shall work out relations
which allow us to determine the constant coefficients $A_\pm$
and $B_\pm$ uniquely.
%
%
\subsubsection{Initial and matching conditions}
%
%
We first use the initial conditions~(\ref{init_cond_on_mu})
in order to fix the constant coefficients $A_\pm$.
\par
For the function $\chi$ such conditions become
%
\be
\lim_{x\rightarrow x_i}\chi(x)
%&=&
=
d\,\sqrt{\frac{1-\epsilon_{1}(x_i)}{2k}}\,
{\rm e}^{-i\,k\,\eta_i-x_i/2}
%\nonumber\\ &=&
=
d\,\sqrt{\frac{1-\epsilon_{1}(x_i)}{2k}}\,
{\rm e}^{i\,\xi_{\rm I}(x_i)-x_i/2}
\ ,
\label{init_cond_on_chi}
\ee
where, from the definitions of $\eta$ and $x$,
$k\,\eta_i\simeq -i\,\xi_{\rm I}(x_i)$.
%
We then recall the asymptotic form of the Bessel functions $J_\nu$
for $x\to+\infty$~\cite{abram,schiff}~\footnote{Since the initial
conditions must be imposed at $x$ in deep region~I,
we can consider $x_i\sim+\infty$.},
%
\be
J_{\pm m}\left[\xi_{\rm I}(x)\right]
\sim
\sqrt{\frac{2}{\pi\,\xi_{\rm I}(x)}}
\,\cos\left(\xi_{\rm I}(x)\mp\frac{\pi}{2}\,m-\frac{\pi}{4}\right)
\ ,
\label{J_asymp}
\ee
%
from which we obtain the asymptotic expression of the mode
function in region~I,
%
{\footnotesize
\be
&&\!\!\!\!\!\!\!\!\chi_{\rm I}(x_i)\!\sim\!
\sqrt{\frac{1-\epsilon_{1}(x_i)}{2\,\pi}}\,{\rm e}^{-{x_i}/{2}}\,\times
\label{init_sol in_I}
\\
&&\!\!\!\!\!\!\!\!\left\{{\rm e}^{+i\,\xi_{\rm I}(x_i)}
\,\left[{\rm e}^{-i\,\left(\frac{1}{4}+\frac{m}{2}\right)\,\pi}\,A_{+}
+{\rm e}^{-i\,\left(\frac{1}{4}-\frac{m}{2}\right)\,\pi}
\left(A_{-}+\varepsilon\,A_{-}\,J_{+-}^{-}(x_0,x_i)
+\varepsilon\,A_{+}\,J_{++}^{+}(x_0,x_i)\right)
\right]\right.
\nonumber
\\
&&\!\!\!\!\!\!\!\!\left.+{\rm e}^{-i\,\xi_{\rm I}(x_i)}\,
\left[{\rm e}^{+i\,\left(\frac{1}{4}+\frac{m}{2}\right)\,\pi}\,A_+
+{\rm e}^{+i\,\left(\frac{1}{4}-\frac{m}{2}\right)\,\pi}\,
\left(A_{-}+\varepsilon\,A_{-}\,J_{+-}^{-}(x_0,x_i)
+\varepsilon\,A_{+}\,J_{++}^{+}(x_0,x_i)\right)
\right]
\right\}
\nonumber
\ .
\ee
}
%
The initial conditions~(\ref{init_cond_on_chi}) therefore yield
%
\be
&&
\!\!\!\!\!\!
A_{+}
=d\,\sqrt{\frac{\pi}{k}}\,
\frac{{\rm e}^{+i\,\left(\frac{1}{4}+\frac{m}{2}\right)\,\pi}}
{1-{\rm e}^{2\,i\,m\,\pi}}
\ ,\
A_{-}
=-A_{+}\,\displaystyle\frac{{\rm e}^{+i\,m\,\pi}
+\varepsilon\,J_{++}^{+}(x_0,x_i)}
{1+\varepsilon\,J_{+-}^{-}(x_0,x_i)}
\ .
\label{A+-}
\ee
Note that $A_+$ does not depend on $\varepsilon$, so it holds to all orders.
\par
We next impose continuity at the turning point in order to determine
the coefficients $B_\pm$.
For this we shall need the (asymptotic) expressions of Bessel functions
for $x\to x_0$~\cite{abram,schiff}~\footnote{The Bessel functions are
actually regular around $x=x_0$, therefore the following expressions
are just the leading terms in the Taylor expansion of $J_\nu$ and $I_\nu$.}.
In particular,
\be
\begin{array}{ll}
J_{\pm m}\left[\xi_{\rm I}(x)\right]
\simeq
\displaystyle
\left[\frac{\xi_{\rm I}(x)}{2}\right]^{\pm m}\,
\frac{1}{\Gamma\left(1\pm m\right)}
&
{\rm for}\
x\to x_0^+
\\
\\
I_{\pm m}\left[\xi_{\rm II}(x)\right]
\simeq
\displaystyle
\left[\frac{\xi_{\rm II}(x)}{2}\right]^{\pm m}\,
\frac{1}{\Gamma\left(1\pm m\right)}
&
{\rm for}\
x\to x_0^-
\ ,
\end{array}
\label{JI_taylor}
\ee
%\end{subequations}
where $\Gamma$ is Euler's gamma function.
Near the turning point, we just keep the leading term in the
expansion~(\ref{omega_expand}), so that
%
\be
&&
\omega(x)\simeq\displaystyle
\sqrt{C}\,\left|x-x_0\right|^{\frac{1-2\,m}{2\,m}}
\ ,\
\xi(x)\simeq
2\,m\,{\sqrt{C}}\,\left|x-x_0\right|^{\frac{1}{2\,m}}
\ .
\label{DX_TP}
\ee
%
We thus obtain the following forms of the mode functions near
the turning point,
\begin{subequations}
%
\be
\!\!\!\!
\chi_{\rm I}(x\simeq x_0)\!\!&\simeq&\!\!
A_{+}\,a_+(x_0)\,
\frac{\sqrt{2\,m}\,\left(m\,\sqrt{C}\right)^{m}}
{\Gamma\left(1+m\right)}\,
\left(x-x_0\right)
\nonumber
\\
&&
\!\!\!\!
+A_{-}\,a_-(x_0)\,
\frac{\sqrt{2\,m}\,\left(m\,\sqrt{C}\right)^{-m}}
{\Gamma\left(1-m\right)}
\label{sol_IX_at_TP}
\\
\phantom{A}
\nonumber
\\
\!\!\!\!\!\!\!\!
\chi_{\rm II}(x\simeq x_0)\!\!&\simeq&\!\!
B_{+}\,b_+(x_0)\,
\frac{\sqrt{2\,m}\,\left(m\,\sqrt{C}\right)^{m}}
{\Gamma\left(1+m\right)}\,
\left(x_0-x\right)
\nonumber
\\
&&
\!\!\!\!
+B_{-}\,b_-(x_0)\,
\frac{\sqrt{2\,m}\,\left(m\,\sqrt{C}\right)^{-m}}
{\Gamma\left(1-m\right)}
\ .
\label{sol_IIX_at_TP}
\ee
\end{subequations}
Continuity across $x_0$ then implies that
\be
B_{+}\,b_+(x_0)=
-A_{+}\,a_+(x_0)
\ ,\ \
B_{-}\,b_-(x_0)=
A_{-}\,a_-(x_0)
\label{connection_at_TP}
\ .
%\end{array}
\ee
%
From the definitions~(\ref{Abar_Bbar}) at $x=x_0$,
Eqs.~(\ref{A+-}) and the relations~(\ref{connection_at_TP})
we therefore obtain
%
\be
\frac{B_{+}}{A_+}&\!\!=\!\!&
-1
+\varepsilon\,
\frac{{\rm e}^{+i\,m\,\pi}
+\varepsilon\,J_{++}^{+}(x_0,x_i)}
{1+\varepsilon\,J_{+-}^{-}(x_0,x_i)}\,
J_{--}^{-}(x_0,x_i)
%\nonumber\\&&
-\varepsilon\,J_{+-}^{+}(x_0,x_i)
\nonumber
\\
\label{B+-}
\\
\frac{B_{-}}{A_+}&\!\!=\!\!&
-\frac{{\rm e}^{+i\,m\,\pi}
+\varepsilon\,J_{++}^{+}(x_0,x_i)}
{1+\varepsilon\,J_{+-}^{-}(x_0,x_i)}
%\nonumber\\&&\ \ \times
\frac{1-i\,\varepsilon^2\,J_{--}^{-}(x_0,x_i)\,
I_{++}^{+}(x_f,x_0)}
{1-i\,\varepsilon\,I_{+-}^{-}(x_f,x_0)}
\nonumber
\\
&&
-i\,\varepsilon\,
\displaystyle\frac{1+\varepsilon\,J_{+-}^{+}(x_0,x_i)}
{1-i\,\varepsilon\,I_{+-}^{-}(x_f,x_0)}\,I_{++}^{+}(x_f,x_0)
\ .
\nonumber
\ee
\par
It is apparent from the above derivation that, since the matching
between approximate solutions in the two regions is always
performed at $x=x_0$, no ambiguity hinders the evaluation of
the coefficients $B_\pm$ and the accuracy of the approximate
solution is therefore expected to increase with increasing order.
%
%
%
\subsubsection{Recursive (perturbative) relations}
%
We can finally obtain expressions for the coefficients
${a}_{\pm}(x)$ and ${b}_{\pm}(x)$ by solving the integral
relations (\ref{Abar_Bbar}).
We remark that the r.h.s.'s of such equations contain
$a_\pm(x)$ and $b_\pm(x)$, which can therefore be determined
recursively by expanding them (as well as any function of them)
in $\varepsilon$, that is
\be
a_\pm(x)=1+\displaystyle\sum_{q\geq1} \varepsilon^q\,a_{\pm}^{(q)}\ ,\ \
b_\pm(x)=1+\displaystyle\sum_{q\geq1} \varepsilon^q\,b_{\pm}^{(q)}
\ .
\ee
It will also be useful to define the following integrals
%\begin{subequations}
\be
&&
\!\!\!\!\!\!\!\!\!\!
J^{w(q)}_{s\bar s}(x_1,x_2)\equiv
\displaystyle\frac{\pi}{\sqrt{3}}\,
\int_{x_1}^{x_2}\!\!\!
\sigma_{\rm I}(y)\,a_w^{(q)}(y)\,
u_{Is}(y)\,u_{I\bar s}(y)\,\d y
\nonumber
\\
\\
&&
\!\!\!\!\!\!\!\!\!\!
I^{w(q)}_{s\bar s}(x_1,x_2)\equiv
\displaystyle\frac{\pi}{\sqrt{3}}\,
\int_{x_1}^{x_2}\!\!\!\!
\sigma_{\rm II}(y)\,b_w^{(q)}(y)\,
u_{IIs}(y)\,u_{II\bar s}(y)\,\d y
\,,
\nonumber
\ee
where again $w$, $s$ and $\bar s=\pm$, and $q$ is a
non-negative integer.\\
\\
%
%
%
%
%
{\em Leading order}\\
\\
%
We begin by considering the leading~($\varepsilon^0$) order
\be
a_\pm^{(0)}(x)=b_\pm^{(0)}(x)=1
\ .
\label{0-th}
\ee
The corresponding solutions are simply given by
\begin{subequations}
%
\be
&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
\chi_{\rm I}(x)\simeq
u_{\rm I}(x)
=A_+\,\sqrt{\frac{\xi_{\rm I}(x)}{\omega_{\rm I}(x)}}\,
\left\{
J_{+m}\left[\xi_{\rm I}(x)\right]
-\,{\rm e}^{+i\,m\,\pi}\,J_{-m}\left[\xi_{\rm I}(x)\right]
\right\}
\label{sol_in_I_leading}
\\
\nonumber
\\
&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
\chi_{\rm II}(x)\simeq
u_{\rm II}(x)
=-A_+\,\sqrt{\frac{\xi_{\rm II}(x)}{\omega_{\rm II}(x)}}\,
\left\{
\,I_{+m}\left[\xi_{\rm II}(x)\right]
+{\rm e}^{+i\,m\,\pi}\,I_{-m}\left[\xi_{\rm II}(x)\right]
\right\}
\label{sol_in_II_leading}
\ ,
\ee
\end{subequations}
%
where we used the zero~order forms of
Eqs.~(\ref{A+-}) and~(\ref{B+-}),
%
\be
A_{-}=B_{-}=-A_{+}\,{\rm e}^{+i\,m\,\pi}
\ ,\ \
B_{+}=-A_{+}
\ .
\label{relation_AB_leading}
\ee
%
\par
We know that these expressions are also good solutions
of Eq.~(\ref{new_eq}) near the turning point and,
deep in region~II, we can use the asymptotic form of
$I_\nu$ for $x\sim x_f\to -\infty$~\cite{schiff,abram},
%
\be
I_{\pm m}\left[\xi_{\rm II}(x)\right]
&\!\!\sim\!\!&
\frac{1}{\sqrt{2\,\pi\,\xi_{\rm II}(x)}}\,
\left[{\rm e}^{\xi_{\rm II}(x)}
+{\rm e}^{-\xi_{\rm II}(x)-i\,\left(\frac12\pm m\right)\,\pi}\right]
\ .
\label{I_asymp}
\ee
%
On neglecting the non-leading mode ${\rm e}^{-\xi_{\rm II}(x)}$,
we then obtain
%
\be
\chi_{\rm II}(x_f)\sim
-A_{+}
\,\frac{\left(1+{\rm e}^{+i\,m\,\pi}\right)}
{\sqrt{2\,\pi\,\omega_{\rm II}(x_f)}}
\,{\rm e}^{\xi_{\rm II}(x_f)}
\ .
\label{sol_deep_in II}
\ee
%
If we now use Eqs.~(\ref{spectra_def}),~(\ref{A+-})
and~(\ref{sol_deep_in II}), and the values of $d$,
we recover the results of Ref.~\cite{martin_schwarz2}
for all quantities of interest,
i.e.~power spectra, spectral indices and
$\alpha$-runnings
%
\begin{subequations}
%
\be
&&
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
{\cal P}_{\zeta}
\simeq
\frac{H^2}{\pi\,\epsilon_1\,m_{\rm Pl}^2}
\left(\frac{k}{a\,H}\right)^3
\frac{{\rm e}^{2\,\xi_{{\rm II,S}}(k,\eta)}}
{\left[1-\epsilon_1(\eta)\right]\,\omega_{\rm II,S}(k,\eta)}
\equiv{\cal P}_{\zeta}^{(0)}
\label{spectra_S_M&S}
\\
\nonumber
\\
&&
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
n_{\rm S}-1\simeq
3+2\,\left.\frac{\d\,\xi_{{\rm II,S}}}{\d\,\ln k}
\right|_{k=k_*}
\label{indices_S_M&S}
\\
\nonumber
\\
&&
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
\alpha_{\rm S}\simeq
2\,\left.
\frac{\d^2\,\xi_{{\rm II,S}}}{\left(\d\,\ln k\right)^2}
\right|_{k=k_*}
\ ,
\label{runnings_S_M&S}
\ee
and
\be
&&
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
{\cal P}_{h}\simeq
\frac{16\,H^2}{\pi\,m_{\rm Pl}^2}
\,\left(\frac{k}{a\,H}\right)^3\,
\frac{{\rm e}^{2\,\xi_{{\rm II,T}}(k,\eta)}}
{\left[1-\epsilon_1(\eta)\right]\,\omega_{\rm II,T}(k,\eta)}
\equiv{\cal P}_{h}^{(0)}
\label{spectra_T_M&S}
\\
\nonumber
\\
&&
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
n_{\rm T}\simeq
3+2\,\left.\frac{\d\,\xi_{{\rm II,T}}}{\d\,\ln k}
\right|_{k=k_*}
\label{indices_T_M&S}
\\
\nonumber
\\
&&
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
\alpha_{\rm T}\simeq
2\,\left.\frac{\d^2\,\xi_{{\rm II,T}}}{\left(\d\,\ln k\right)^2}
\right|_{k=k_*}
\ ,
\label{runnings_T_M&S}
\ee
\end{subequations}

%
where we have transformed back to the original
variables $k$ and $\eta$, and all quantities are
evaluated in the super-horizon limit (i.e.~for
$k\ll a\,H$).\\
\\
%
%
%
%
%
{\em Next-to-leading order}\\
\\
%
We now insert the leading order expressions~(\ref{0-th})
into the integral relations~(\ref{Abar_Bbar}) to compute the
next-to-leading order expressions
%\begin{subequations}
%
\be
&&
{a}_{+}^{(1)}(x)=
J_{+-}^{(0)}(x,x_i)
-{\rm e}^{+i\,m\,\pi}\,J^{(0)}_{--}(x,x_i)
\nonumber %\label{a+_tilde_1}
\\
\nonumber
\\
&&
{a}_{-}^{(1)}(x)=
J^{(0)}_{+-}(x_0,x)
-{\rm e}^{-i\,m\,\pi}\,J^{(0)}_{++}(x_0,x)
\nonumber %\label{a-_tilde_1}
\\
\label{ab+-1}
\\
&&
{b}_{+}^{(1)}(x)=
-i\,I^{(0)}_{+-}(x,x_0)
-i\,{\rm e}^{+i\,m\,\pi}\,I^{(0)}_{--}(x,x_0)
\nonumber %\label{b+_tilde_1}
\\
\nonumber
\\
&&
{b}_{-}^{(1)}(x)=
-i\,I^{(0)}_{+-}(x_f,x)
-i\,{\rm e}^{-i\,m\,\pi}\,I^{(0)}_{++}(x_f,x)
\ ,
\nonumber %\label{b-_tilde_1}
\ee
%\end{subequations}
%
where we used the simplified notation
$J^{+(0)}_{s\bar s}=J^{-(0)}_{s\bar s}\equiv J^{(0)}_{s\bar s}$
and $I^{+(0)}_{s\bar s}=I^{-(0)}_{s\bar s}\equiv I^{(0)}_{s\bar s}$,
and also expanded the coefficients $A_-$ and $B_\pm$ to zero
order in $\varepsilon$.
\par
From Eq.~(\ref{I_asymp}), again neglecting the non-leading mode
${\rm e}^{-\xi_{\rm II}(x)}$, we obtain the mode function
at $x=x_f$ to first order in $\varepsilon$,
%
\be
&&\!\!\!\!\!\!\!\!\!\!
\chi_{\rm II}(x_f)\!\sim\!
-\frac{A_+\,{\rm e}^{\xi_{\rm II}(x_f)}}
{\sqrt{2\,\pi\,\omega_{\rm II}(x_f)}}\,
\left\{1+{\rm e}^{+i\,m\,\pi}
%\phantom{\frac{A}{B}}
\right.
%\nonumber\\&&\ \ \
+i\,\varepsilon\,
\left[I_{++}^{(0)}(x_f,x_0)-I_{+-}^{(0)}(x_f,x_0)\right]
\nonumber
\\
&&\!\!\!\!\!\!\!\!
-i\,\varepsilon\,{\rm e}^{+i\,m\,\pi}\,
\left[I_{--}^{(0)}(x_f,x_0)-I_{+-}^{(0)}(x_f,x_0)\right]
%\nonumber\\&&\ \ \
-\varepsilon\,{\rm e}^{+i\,m\,\pi}\,
\left[J_{+-}^{(0)}(x_0,x_i)+J_{--}^{(0)}(x_0,x_i)\right]
\nonumber
\\
&&\!\!\!\!\!\!\!\!
\left.
+\varepsilon\left[J_{+-}^{(0)}(x_0,x_i)+J_{++}^{(0)}(x_0,x_i)\right]
\right\}
\ ,
\label{sol_deep_in II_next_leading}
\ee
%
%
which, using Eqs.~(\ref{spectra_def}), (\ref{A+-}),
(\ref{sol_deep_in II_next_leading}) and the values of $d$,
yields all quantities of interest to first order in
$\varepsilon$.
For the spectra we obtain
\be
{\cal P}_{\zeta}\simeq
{\cal P}_{\zeta}^{(0)}\,
\left[1+g_{(1) \, {\rm S}}^{\rm GREEN} (x_f)\right]
\ ,\ \
{\cal P}_{h}\simeq
{\cal P}_{h}^{(0)}\,
\left[1+g_{(1) \, {\rm T}}^{\rm GREEN} (x_f)\right]
\ ,
\label{spectra_next-to-leading}
\ee
where the relative corrections to the leading order
expressions~(\ref{spectra_S_M&S}) and~(\ref{spectra_T_M&S})
are now given by
\be
&&
\!\!\!\!\!\!\!\!
g_{(1) \, {\rm S,T}}^{\rm GREEN} (x)=
\left\{
J_{++}^{(0)}(x_0,x_i)-J_{--}^{(0)}(x_0,x_i)
\right.
\nonumber
\\
&&
\!\!\!\!\!\!\!\!
\left.
+\frac{1}{\sqrt{3}}
\left[I_{++}^{(0)}(x,x_0)
-2\,I_{+-}^{(0)}(x,x_0)
+I_{--}^{(0)}(x,x_0)\right]
\right\}_{\rm S,T}
\ ,
\label{g(1)}
\ee
in which we set $\varepsilon=1$ and $n=1$ as required, and
write S and T to recall the use of the corresponding
frequencies.
The expressions for the spectral indices and their runnings
to this order can finally be derived from the
definitions~(\ref{n_def}) and~(\ref{alpha_def}).\\
\\
%
%
%
%
{\em Higher orders}\\
\\
%
The above procedure can be extended to all orders.
The coefficients up to $a_\pm^{(q)}$ and $b_\pm^{(q)}$ must
be used to compute the integrals $J^{w(q)}_{s\bar s}$ and
$I^{w(q)}_{s\bar s}$ which determine $a_\pm^{(q+1)}$ and
$b_\pm^{(q+1)}$.
However, general expressions soon become very involved,
and we shall test the effectiveness of our method by
applying it to several cases of interest.
%
%
%
\subsection{Adiabatic expansion}
\label{adiab}
%
Let us now apply the usual adiabatic expansion with the
assumption that the leading order be given by the
functions~(\ref{particular_sol})
[rather than the more common expression~(\ref{wkb_sol})].
This leads one to replace
\be
\xi(x)\to
\frac{\xi(x)}{\sqrt{\delta}}
\equiv\frac{1}{\sqrt{\delta}}\,\int^x
\omega(y)\,\d y
\ ,
\ee
and consider the forms~\cite{langer}.
\begin{subequations}
\be
U_\pm=F_\pm(x;\delta)\,u_\pm(x)+G_\pm(x;\delta)\,u'_\pm(x)
\ ,
\ee
where the $x$-dependent coefficients $F$ and $G$ must now
be determined.
The particular case of a linear turning
point~\cite{langer49}
(precisely the one which mostly concerns us here),
can then be fully analyzed as follows.
%
%
\subsubsection{Recursive (adiabatic) relations}
%
%
The $x$-dependent coefficients $F$ and $G$ can be
expanded in powers of $\delta$ as
\be
&&
F(x;\delta)=\sum_{j\ge 0} \delta^j\,\phi_{(j)}(x)
\nonumber
\\
\label{adiab_exp}
\\
&&
G(x;\delta)=\sum_{j\ge 0} \delta^j\,\gamma_{(j)}(x)
\nonumber
\ .
\ee
Upon substituting into Eq.~(\ref{new_eq_rewrite}) with
$\varepsilon=1$, one therefore obtains that the coefficients
$\phi_{(j)}$ and $\gamma_{(j)}$ are given recursively
by the formulae
\be
\phi_{(j)}(x)&\!\!=\!\!&-\frac{1}{2}
\int^{x}
\left[\gamma''_{(j)}(y)+\sigma(y)\,\gamma_{(j)}(y)\right]
\d y
\nonumber
\\
\label{delta_j}
\\
\gamma_{(j)}(x)&\!\!=\!\!&\frac{1}{2\,\omega(x)}
\int^x
\!\!
\left\{
\sigma(y)\,\left[2\,\gamma'_{(j-1)}(y)+\phi_{(j-1)}(y)\right]
%\,\frac{\d y}{\omega(y)}
\right.
\nonumber
\\
&&
\phantom{\frac{1}{2\,\omega(x)}\,\int\!\!\!}
\left.
+\sigma'(y)\,\gamma_{(j-1)}(y)+\phi''_{(j-1)}(y)\right\}
\frac{\d y}{\omega(y)}
\ ,
\nonumber
\ee
\end{subequations}
where it is understood that the integration must be performed
from $x_0$ to $x$ in region~I and from $x$ to $x_0$ in region~II.
Let us also remark that, for $\omega^2\sim (x-x_0)$ near the
turning point, the above expressions are finite~\cite{langer49},
whereas for more general cases one expects divergences as
with the more standard WKB approach.\\
\\
%
%
{\em Leading order}\\
\\
%
%
The lowest order solutions (\ref{particular_sol}) are correctly
recovered on setting
\be
\phi_{(0)}=1
\quad
{\rm and}
\quad
\gamma_{(0)}=0
\ ,
\label{delta0}
\ee
in the limit $\delta=1$.
The relevant leading order perturbations are therefore obtained
on imposing the initial conditions~(\ref{init_cond_on_chi})
and matching conditions between region~I and region~II at the
turning point, which therefore yield for $\chi_{\rm I}$ and
$\chi_{\rm II}$ the same linear combinations $u_{\rm I}$
of Eq.~(\ref{sol_in_I_leading}) and $u_{\rm II}$ of
Eq.~(\ref{sol_in_II_leading}) previously obtained.\\
\\
%
%
{\em Higher orders}\\
\\
%
The condition~(\ref{delta0}) makes the formal expressions of
the coefficients $\phi_{(1)}$ and $\gamma_{(1)}$ particularly
simple,
\be
\phi_{(1)}(x)&\!\!=\!\!&-\frac{1}{2}\,\int^{x}
\left[\gamma''_{(1)}(y)+\sigma(y)\,\gamma_{(1)}(y)\right]\,
\d y
\nonumber
\\
\label{delta1}
\\
\gamma_{(1)}(x)&\!\!=\!\!&\frac{1}{2\,\omega(x)}\,\int^x
\frac{\sigma(y)}{\omega(y)}\,
\d y
\ ,
\nonumber
\ee
and the first order solutions are then given by linear combinations
of the two functions
\be
U_\pm(x)=\left[1+\delta\,\phi_{(1)}(x)\right]\,u_\pm(x)
+\delta\,\gamma_{(1)}(x)\,u'_\pm(x)
\ .
\ee
\par
It is now important to observe that the initial conditions~(\ref{init_cond_on_chi}) and matching conditions
at the turning point to first order in the adiabatic
parameter $\delta$ yield different results with respect
to the perturbative expansion in $\varepsilon$.
First of all, the coefficient $A_+$, which was left unaffected
by the expansion in $\varepsilon$ [see~Eq.~(\ref{A+-})],
acquires a correction.
The relations between $A_-$, $B_\pm$ and $A_+$ instead
remain those given in Eq.~(\ref{relation_AB_leading})
to all orders, whereas in the perturbative
expansion they were modified [see Eqs.~(\ref{A+-})
and~(\ref{B+-})].
To summarize, to first order in $\delta$,
one obtains
\be
A_+&\!\!\simeq\!\!&
d\,\sqrt{\frac{\pi}{k}}\,
\frac{{\rm e}^{i\,\left(\frac{1}{4}+\frac{m}{2}\right)\,\pi}}
{1-{\rm e}^{2\,i\,m\,\pi}}\,
\left\{1-\delta\,\left[
\phi_{{\rm I}(1)}(x_i)
+\gamma_{{\rm I}(1)}(x_i)\,\left(
i\,\omega_{\rm I}(x_i)-\frac{1}{2}\right)
\right]\right\}
\nonumber
\\
A_-&\!\!=\!\!&-A_+\,{\rm e}^{+i\,m\,\pi}
\ ,\ \
B_\pm=\mp A_\pm
\ ,
\label{ABadia1}
\ee
and the perturbation modes deep in Region~II
(at $x\ll x_0$) are finally given by
%
%\begin{subequations}
\be
\chi_{\rm II}(x)
\simeq
u_{\rm II}(x)\,
\left\{1+
\delta\,\left[
\phi_{{\rm II}(1)}(x)
-\gamma_{{\rm II}(1)}(x)\,\left(
\omega_{\rm II}(x)
+\frac{\omega_{\rm II}'(x)}{2\,\omega_{\rm II}(x)}\right)
\right.\right.
\nonumber
\\
\left.\left.
-\phi_{{\rm I}(1)}(x_i)
+\gamma_{{\rm I}(1)}(x_i)\,\left(
\frac{1}{2}-i\,\omega_{\rm I}(x_i)\right)
\right]
\right\}
\ .
\label{chi_1}
\ee
We note that, in order to obtain the above result,
one must first take the asymptotic expansion of the
functions $u_\pm$ and then take the derivative,
since the reverse order would lead to larger errors.
The corrected power spectra are then given by
\begin{subequations}
\be
{\cal P}_\zeta\simeq
{\cal P}^{(0)}_\zeta\,\left[1+g_{(1){\rm S}}^{\rm AD}(x_f)
\right]
\ ,\ \
{\cal P}_h\simeq
{\cal P}^{(0)}_h\,\left[1+g_{(1){\rm T}}^{\rm AD} (x_f)\right]
\ ,
\label{spectra_correct}
\ee
in which we set $\delta=1$ at the end~\footnote{Since our method has some similarity with that
of Ref.~\cite{HHHJM} (see also Ref.~\cite{olver}),
it is worth pointing out that the first order corrections
shown here differ from those of Ref.~\cite{HHHJM} (at least)
in that they contain contributions from both Regions~I and~II.}.
The spectral indices are also given by
%
\be
&&
n_{\rm S}-1=
3+2\,
\frac{\d\,\xi_{\rm II,S}}{\d\,\ln k}
+
\frac{\d\,g_{(1){\rm S}}^{\rm AD}}{\d\,\ln k}
\nonumber
\\
\label{index_correct}
\\
&&
n_{\rm T}=
3+2\,
\frac{\d\,\xi_{\rm II,T}}{\d\,\ln k}
+
\frac{\d\,g_{(1){\rm T}}^{\rm AD}}{\d\,\ln k}
\ ,
\nonumber
\ee
%
and their runnings by
%
\be
&&
\alpha_{\rm S}=
2\,
\frac{\d^2\,\xi_{\rm II,S}}{\left(\d\,\ln k\right)^2}
+
\frac{\d^2\,g_{(1){\rm S}}^{\rm AD}}{\left(\d\,\ln k\right)^2}
\nonumber
\\
\label{runnings_correct}
\\
&&
\alpha_{\rm T}=
2\,
\frac{\d^2\,\xi_{\rm II,T}}{\left(\d\,\ln k\right)^2}
+
\frac{\d^2\,g_{(1){\rm T}}^{\rm AD}}{\left(\d\,\ln k\right)^2}
\ .
\nonumber
\ee
%
Finally, the tensor-to-scalar ratio takes the form
%
\be
R=16\,\epsilon_1\,
\frac{{\rm e}^{2\,\xi_{\rm II,T}}\,\left(1+g_{(1){\rm T}}^{\rm AD}\right)\,
\omega_{\rm II,S}}
{{\rm e}^{2\,\xi_{\rm II,S}}\,\left(1+g_{(1){\rm S}}^{\rm AD}\right)\,
\omega_{\rm II,T}}
\ ,
\label{R_correct}
\ee
\end{subequations}
%
where all quantities are evaluated in the super-horizon limit
($x\ll x_0$) and we used the results
{\footnotesize
\be
g_{(1){\rm S,T}}^{\rm AD}(x)
=
%&\!\!\!=\!\!\!&
2\left[
\phi_{{\rm II}(1)}(x)
-\gamma_{{\rm II}(1)}(x)
\left(\omega_{\rm II}(x)
+\frac{\omega_{\rm II}'(x)}{2\,\omega_{\rm II}(x)}\right)
%\right.\nonumber\\&&\left.\phantom{2\,[}
+\frac{\gamma_{{\rm I}(1)}(x_i)}{2}
-\phi_{{\rm I}(1)}(x_i)
\right]_{\rm S,T}
\ ,
\label{g_1}
\ee
}
where the indices S and T recall the use of the
corresponding frequencies.
\par
Given the complicated expressions for $\omega$, it is
usually impossible to carry out the double integration that
yields $\phi_{(1)}$ analytically, let alone higher order terms.
One must therefore rely on numerical computations.
In the context of power-law inflation we can compare results obtained
in next-to-leading order from the two expansions with the exact result.
%
\section{Method of Comparison Equation}
\label{sMCE}
%
Let us briefly review the Method of Comparison Equation - the name is due to Dingle~\cite{dingle} - MCE henceforth.
It was independently introduced in Refs.~\cite{MG,dingle} and
applied to wave mechanics by Berry and Mount in Ref.~\cite{berry}.
The standard WKB approximation and its improvement by Langer~\cite{langer}
are just particular cases of this method and its connection with
the Ermakov-Pinney equation is studied in Appendix~\ref{appKLV}.
\par
We start from the well-known second-order differential equation~(\ref{new_eq})
%
\be
\left[
\frac{{\d}^2}{{\d}x^2}+\omega^2(x)
\right]
\,\chi(x)=0
\ ,
\label{exact_EQ}
\ee
%
where $\omega^2$ is a (not necessarily positive) ``potential''
(or ``frequency''), and suppose that we know an exact solution to a
similar second-order differential equation,
%
\be
\left[
\frac{{\d}^2}{{\d}\sigma^2}+\Theta^2(\sigma)
\right]
\,U(\sigma)=0
\ ,
\label{aux_EQ}
\ee
%
where $\Theta$ is the ``comparison function''.
One can then represent an exact solution of Eq.~(\ref{exact_EQ})
in the form
%
\be
\chi(x)=\left(\frac{{\d}\sigma}{{\d}x}\right)^{-1/2}\,U(\sigma)
\ ,
\label{exact_SOL}
\ee
%
provided the variables $x$ and $\sigma$ are related by
%
\be
\omega^2(x)\!=\!\left(\frac{{\d}\sigma}{{\d}x}\right)^{2}\Theta^2(\sigma)
-\left(\frac{{\d}\sigma}{{\d}x}\right)^{1/2}
\frac{{\d}^2}{{\d}x^2}\left(\frac{{\d}\sigma}{{\d}x}\right)^{-1/2}
\ .
\label{new_EQ}
\ee
%
Eq.~(\ref{new_EQ}) can be solved by using some iterative
scheme, in general cases as~\cite{hecht} and Appendix~\ref{appKLV} or for specific
problems~\cite{mori,pechukas}.
If we choose the comparison function sufficiently similar to
$\omega$, the second term in the right hand side (r.h.s.) of
Eq.~(\ref{new_EQ}) will be negligible with respect to the first
one, so that
%
\be
\omega^2(x)\simeq\left(\frac{{\d}\sigma}{{\d}x}\right)^{2}
\Theta^2(\sigma)
\ .
\label{new_EQ_appr}
\ee
%
On selecting a pair of values $x_0$ and $\sigma_0$ such that
$\sigma_0=\sigma(x_0)$, the function $\sigma(x)$ can be implicitly
expressed as
%
\be
-\xi(x)\equiv
\int_{x_0}^x\sqrt{\pm\,\omega^2(y)}\,{\d}\,y
\simeq
\int_{\sigma_0}^{\sigma}\sqrt{\pm\,\Theta^2(\rho)}\,{\d}\,\rho
\ ,
\label{new_EQ_int}
\ee
%
where the signs are chosen conveniently~\footnote{Here
$\xi(x)$ corresponds to the quantity $\xi_{\rm II}(x)$ used in
Section~\ref{imprWKB} when the signs are both chosen minus.}.
The result in Eq.~(\ref{exact_SOL}) leads to a uniform approximation
for $\chi(x)$, valid in the whole range of the variable $x$, including
``turning points''~\footnote{With this term, borrowed from point
particle mechanics, one usually means a real zero of the ``frequency''
$\omega$.}.
The similarity between $\Theta$ and $\omega$ is clearly very
important in order to implement this method.
%
%
%
%
\par
In order to apply the MCE to cosmological perturbations, we note that
the frequency $\omega^2(x)$ is
%
\be
\omega^2(x)=\frac{{\rm e}^{2\,x}}{\left[1-\epsilon_1(x)\right]^2}-\nu^2(x)
\ ,
\label{our_freq}
\ee
%
with $\nu^2(x)$ given, respectively for scalar and tensor
perturbations, by
%
{\small
\begin{subequations}
\be
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
\nu_{\rm S}^2(x)&=&
\frac{1}{4}\,\left(\frac{3-\epsilon_1}{1-\epsilon_1}\right)^2
+\frac{(3-2\,\epsilon_1)\,\epsilon_2}{2\,(1-\epsilon_1)^2}
%\nonumber\\&&
+\frac{(1-2\,\epsilon_1)\,\epsilon_2\,\epsilon_3}{2\,(1-\epsilon_1)^3}
+\frac{(1-4\,\epsilon_1)\,\epsilon_2^2}{4\,(1-\epsilon_1)^4}
\label{nu2_S}
\\
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
\nu_{\rm T}^2(x)&=&
\frac{1}{4}\,\left(\frac{3-\epsilon_1}{1-\epsilon_1}\right)^2
-\frac{\epsilon_1\,\epsilon_2}{2\,(1-\epsilon_1)^2}
-\frac{\epsilon_1\,\epsilon_2\,\epsilon_3}{2\,(1-\epsilon_1)^3}
-\frac{(2+\epsilon_1)\,\epsilon_1\,\epsilon_2^2}{4\,(1-\epsilon_1)^4}
\ ,
\label{nu2_T}
\ee
\end{subequations}
}
%
where we omit the dependence on $x$ in the $\epsilon_i$ for the sake of
brevity. From Eqs.~(\ref{our_freq}), (\ref{nu2_S}) and (\ref{nu2_T}) we can recognise
our second-order differential basic equations~(\ref{eqST_x}).
The point $x=x_0$ where the frequency vanishes, $\omega(x_0)=0$
(i.e.~the classical ``turning point''), is given by the expression
%
\be
x_0=\ln\left[\bar{\nu}\,\left(1-\bar{\epsilon}_1\right)\right]
\ ,
\ee
%
where we have defined $\bar{\nu}\equiv\nu(x_0)$ and
$\bar{\epsilon}_1\equiv\epsilon_1(x_0)$.
We now choose the comparison function
%
\be
\Theta^2(\sigma)=
\frac{{\rm e}^{2\,\sigma}}{(1-\bar{\epsilon}_1)^2}-\bar{\nu}^2
\ ,
\label{aux_FREQ}
\ee
%
and note that then $\sigma_0=x_0$.
Solutions to Eq.~(\ref{exact_EQ}) can now be expressed, by means of
Eqs.~(\ref{aux_EQ}), (\ref{new_EQ_appr}) and (\ref{aux_FREQ}), as
%
\be
\chi_{\pm}(x)\simeq\sqrt{\frac{\Theta(\sigma)}{\omega(x)}}\,
J_{\pm\bar{\nu}}\left(\frac{{\rm e}^{\sigma}}{1-\bar{\epsilon}_1}\right)
\ ,
\label{exact_SOL_bis}
\ee
%
where the $J$'s are Bessel functions~\cite{abram}, and the
initial condition~(\ref{init_cond_on_mu}) can be satisfied by taking
a linear combination of them.
However, in contrast with the improved WKB method presented in
Section~\ref{imprWKB}, MCE solutions need not be matched at the turning
point, since the functions~(\ref{exact_SOL_bis}) are valid solutions
for the whole range of the variable $x$.
Eq.~(\ref{new_EQ_int}) at the end of inflation, $x=x_{\rm f}$, becomes
%
\be
\xi(x_{\rm f})
&\simeq&
-\Theta(\sigma_{\rm f})
-\frac{\bar{\nu}}{2}\,\ln\left[
\frac{\bar{\nu}-\Theta(\sigma_{\rm f})}
{\bar{\nu}+\Theta(\sigma_{\rm f})}\right]
\nonumber
\\
&\simeq&
-\bar{\nu}\,
\left[1+\ln\left(\frac{{\rm e}^{\sigma_{\rm f}}}{1-\bar{\epsilon}_1}\right)
-\ln\left(2\,\bar{\nu}\right)\right]
\ ,
\label{new_EQ_integrate}
\ee
%
where the super-horizon limit
$x_{\rm f}\ll x_0$ ($\sigma_{\rm f}\to-\infty$)
has been taken in the second line.
One then has
%
\be
\frac{{\rm e}^{\sigma_{\rm f}}}{1-\bar{\epsilon}_1}
\simeq
\frac{2\,\bar{\nu}}{\rm e}\,{\rm exp}
\left[-\frac{\xi(x_{\rm f})}{\bar{\nu}}\right]
\ .
\label{arg_exp}
\ee
%
Finally, on using Eq.~(\ref{arg_exp}), we obtain the general expressions
for the power spectra to leading MCE order,
%
\begin{subequations}
\be
{\cal P}_\zeta
&=&
\left[\frac{H^2}{\pi\,\epsilon_1\,m_{\rm Pl}^2}
\left(\frac{k}{a\,H}\right)^3
\frac{{\rm e}^{2\,\xi_{\rm S}}}
{\left(1-\epsilon_1\right)\,\omega_{\rm S}}\right]_{x=x_{\rm f}}
g_{\rm S}(x_0)
\label{spectra_S}
\\
{\cal P}_h
&=&
\left[\frac{16\,H^2}{\pi\,m_{\rm Pl}^2}\,
\left(\frac{k}{a\,H}\right)^3\,
\frac{{\rm e}^{2\,\xi_{\rm T}}}
{\left(1-\epsilon_1\right)\,\omega_{\rm T}}\right]_{x=x_{\rm f}}
g_{\rm T}(x_0)
\label{spectra_T}
\ ,
\ee
%
where $m_{\rm Pl}$ is the Planck mass and the quantities inside the
square brackets are evaluated in the super-horizon limit, whereas
the functions
%
\be
g(x_0)
\equiv
\frac{\pi\,e^{2\,\bar{\nu}}\,\bar{\nu}^{1-2\,\bar{\nu}}}
{\left[1-\cos\left(2\,\pi\,\bar{\nu}\right)\right]\,
\left[\Gamma\left(1-\bar{\nu}\right)\right]^2}
\ ,
\label{corr_TP}
\ee
\end{subequations}
%
describe corrections that just depend on quantities evaluated
at the turning point and represent the main result of the
MCE applied to cosmological perturbations~\footnote{Inside the
square brackets we recognize the general results ${\cal P}_{\zeta}^{(0)}$
and ${\cal P}_{h}^{(0)}$ given by the WKB (leading-order) approximation
in Section~\ref{imprWKB}.
The ``correction'' $g(x_0)$ accounts for the fact that $\Theta^2$
in Eq.~(\ref{aux_FREQ}) is a better approximation than
Langer's~\cite{WKB1,langer}.}.
The expression in Eq.~(\ref{corr_TP}) is obtained by simply making use of
the approximate solutions~(\ref{exact_SOL_bis}) and their asymptotic
expansion at $x\to\infty$ to impose the initial
conditions~(\ref{init_cond_on_mu}).
In Section~\ref{imprWKB} one finds a similar
factor but, in that case, using the Bessel functions of order $1/3$ leads
to a large error in the amplitudes.
The MCE instead uses Bessel functions of order $\bar{\nu}$, with $\bar\nu=3/2$
to leading order in the HFF (i.e.~the right index for the de~Sitter model),
which yields a significantly better value for the amplitudes of inflationary
spectra.
\par
The MCE allows one to compute approximate perturbation modes with errors
in the asymptotic regions (i.e.~in the sub- and super-horizon limits)
which are comparable with those of the standard (or improved) WKB
approximation (see Sec.~\ref{stWKB}).
Since these methods usually give large errors at the turning
point (which produce equally large errors in
the amplitude of the power spectra) it will suffice to estimate the
error at the turning point in order to show that the MCE is indeed
an improvement.
To leading order (that is, on using the approximate
solution~(\ref{exact_SOL_bis})), the MCE gives an error at the
turning point of the second order in the HFF, which means that we
have a small error in the amplitudes of the power spectra.
Unfortunately, this error remains of second order
in the HFF also for next-to-leading order in the MCE.
We shall see this by applying Dingle's analysis~\cite{dingle}
for linear frequencies to our case~(\ref{our_freq}).
We start by rewriting Eq.~(\ref{new_EQ}) as
%
\be
\left\{\omega^2-\sigma_1^2\,\left[\frac{{\rm e}^{2\,\sigma}}
{(1-\bar{\epsilon}_1)^2}-\bar{\nu}^2\right]
\right\}
+
\left[
\frac34\,\frac{\sigma_2^2}{\sigma_1^2}-\frac12\,\frac{\sigma_3}{\sigma_1}
\right]
=0
\ ,
\label{new_EQ_4_DING}
\ee
%
where we dropped the $x$ dependence in $\omega$ and $\sigma$
and the order of the derivatives is given by their subscripts
($\sigma_1\equiv \d\sigma/\d x$, $\omega_1^2\equiv \d\omega^2/\d x$,
etc.).
Note that the term in square brackets is the error obtained on using
the solutions~(\ref{exact_SOL_bis}).
We then evaluate Eq.~(\ref{new_EQ_4_DING}) and its subsequent
derivatives at the turning point (i.e.~at $x=x_0$),
%
\begin{subequations}
\be
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
\left\{
\omega^2-\sigma_1^2\,\Theta^2\left(\sigma\right)
\right\}
+
\left[
\frac34\,\frac{\sigma_2^2}{\sigma_1^2}-\frac12\,\frac{\sigma_3}{\sigma_1}
\right]
=0
\label{new_EQ_4_DING_TP}
\ee
%
{\footnotesize
\be
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
\left\{
\omega^2_1
-2\,\sigma_2\,\sigma_1\,\Theta^2\left(\sigma\right)
-\frac{2\,{\rm e}^{2\,\sigma}\,\sigma_1^3}{\left(1-\bar{\epsilon}_1\right)^2}
\right\}
+
\left[
2\,\frac{\sigma_3\,\sigma_2}{\sigma_1^2}
-\frac32\,\frac{\sigma_2^3}{\sigma_1^3}
-\frac12\,\frac{\sigma_4}{\sigma_1}
\right]
=0
\label{new_EQ_deriv1}
\ee
%
\be
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
&&
\left\{
\omega^2_2
-2\,\left(\sigma_3\,\sigma_1+\sigma_2^2\right)\,\Theta^2\left(\sigma\right)
-\frac{2\,\sigma_1^2\,{\rm e}^{2\,\sigma}}{\left(1-\bar{\epsilon}_1\right)^2}\,
\left(2\,\sigma_1^2+5\,\sigma_2\right)
\right\}
\nonumber\\
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
&&
+
\left[
\frac92\,\frac{\sigma_2^4}{\sigma_1^4}
-\frac{17}{2}\frac{\sigma_3\,\sigma_2^2}{\sigma_1^3}
+\frac52\,\frac{\sigma_4\,\sigma_2}{\sigma_1^2}
+2\,\frac{\sigma_3^2}{\sigma_1^2}
-\frac12\,\frac{\sigma_5}{\sigma_1}
\right]
=0
\label{new_EQ_deriv2}
\ee
%
\be
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
&&
\left\{
\omega^2_3
-2\,\left(\sigma_4\,\sigma_1+3\,\sigma_2\,\sigma_3\right)\,\Theta^2\left(\sigma\right)
-\frac{2\,\sigma_1\,{\rm e}^{2\,\sigma}}{\left(1-\bar{\epsilon}_1\right)^2}\,
\left(4\,\sigma_1^4
+18\,\sigma_2\,\sigma_1^2
+7\,\sigma_3\,\sigma_1
+12\,\sigma_2^2\right)
\right\}
\nonumber
\\
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
&&
+\left[
\frac{87}{2}\,\frac{\sigma_3\,\sigma_2^3}{\sigma_1^4}
-18\,\frac{\sigma_2^5}{\sigma_1^5}
-\frac{27}{2}\,\frac{\sigma_4\,\sigma_2^2}{\sigma_1^3}
-21\,\frac{\sigma_3^2\,\sigma_2}{\sigma_1^3}
+3\,\frac{\sigma_5\,\sigma_2}{\sigma_1^2}
+\frac{13}{2}\,\frac{\sigma_3\,\sigma_4}{\sigma_1^2}
-\frac12\,\frac{\sigma_6}{\sigma_1}
\right]
=0
\ ,
\label{new_EQ_deriv3}
\ee
}
\end{subequations}
%
where $\Theta^2\left(\sigma\right)$ was defined in Eq.~(\ref{aux_FREQ})
and we omit two equations for brevity.
In order to evaluate the error at the turning point
\be
\Delta_{\rm TP}=
\left[\frac34\,\frac{\sigma_2^2}{\sigma_1^2}
-\frac12\,\frac{\sigma_3}{\sigma_1}\right]_{x=x_0}
\ ,
\ee
we ignore the terms in square brackets and equate to zero the
expressions in the curly brackets in
Eqs.~(\ref{new_EQ_4_DING_TP})-(\ref{new_EQ_deriv3}) and so on.
This leads to
%
{\small
\begin{subequations}
\be
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
\sigma
&\!=\!&
\ln\left[\left(1-\bar{\epsilon}_1\right)\,\bar{\nu}\right]
\label{sigma0_0order}
\\
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
\sigma_1
&\!=\!&
\left(\frac{\omega^2_1}{2\,\bar{\nu}^{2}}\right)^{1/3}
\label{sigma1_0order}
\\
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
\sigma_2
&\!=\!&
\frac{1}{5\,\left(2\,\bar{\nu}^2\right)^{1/3}}
\left[
\frac{\omega^2_2}{\left(\omega^2_1\right)^{2/3}}
-\left(2\,\frac{\omega^2_1}{\bar{\nu}}\right)^{2/3}
\right]
\label{sigma2_0order}
\\
\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!
\sigma_3
&\!=\!&
-\frac{6 \left(2^{1/3}\,\omega^2_2\right)^2}
{175\,\left(\bar{\nu}^{2/5}\,\omega^2_1\right)^{5/3}}
-\frac{3\cdot 2^{1/3}\,\omega^2_2}
{25\,\left(\bar{\nu}^{4}\,\omega^2_1\right)^{1/3}}
+\frac{16\,\omega^2_1}{175\,\bar{\nu}^2}
+\frac{\omega^2_3}
{7 \left(2^{1/2}\,\bar{\nu}\,\omega^2_1\right)^{2/3}}
\ ,
\label{sigma3_0order}
\ee
\end{subequations}
}
%
and similar expressions for $\sigma_4$, $\sigma_5$, and $\sigma_6$
which we again omit for brevity.
On inserting Eqs.~(\ref{our_freq}), (\ref{nu2_S}) and (\ref{nu2_T})
in the above expressions, we find the errors to leading MCE order
%
\begin{subequations}
\be
\Delta^{(0)}_{\rm TP, S}&=&
-\frac{32}{315}\,\epsilon_1\,\epsilon_2
-\frac{22}{315}\,\epsilon_2\,\epsilon_3
\label{corr_TP_S_0order}
\\
\Delta^{(0)}_{\rm TP, T}&=&
-\frac{32}{315}\,\epsilon_1\,\epsilon_2
\ ,
\label{corr_TP_T_0order}
\ee
\end{subequations}
for scalar and tensor modes respectively.
%
\par
On iterating this procedure we can further obtain the errors
for the next-to-leading MCE order $\Delta^{(1)}_{\rm TP}$.
We first compute next-to-leading solutions to
Eqs.~(\ref{new_EQ_4_DING_TP})-(\ref{new_EQ_deriv3}) and so on
by inserting the solutions found to leading order for
$\sigma_1,\sigma_2,\ldots,\sigma_6$ into the corrections
(i.e.~the square brackets) and into all terms containing
$\Theta^2(\sigma)$~\cite{dingle}.
This leads to
%
\begin{subequations}
\be
\Delta^{(1)}_{\rm TP, S}&=&
-\frac{31712}{331695}\,\epsilon_1\,\epsilon_2
-\frac{21598}{331695}\,\epsilon_2\,\epsilon_3
\label{corr_TP_S_1order}
\\
\Delta^{(1)}_{\rm TP, T}&=&
-\frac{31712}{331695}\,\epsilon_1\,\epsilon_2
\ ,
\label{corr_TP_T_1order}
\ee
\end{subequations}
%
which show that the next-to-leading MCE solutions lead to an error of
second order in the HFF, too.
We suspect that this remains true for higher MCE orders, since there
is no {\em a priori\/} relation between the MCE and the
slow-roll expansions.
Let us however point out that the above expressions were obtained
without performing a slow-roll expansion and therefore do not
require that the $\epsilon_i$ be small.
%
%
%
%

